DeepASL: Enabling Ubiquitous and Non-Intrusive Word and Sentence-Level Sign Language Translation

There is an undeniable communication barrier between deaf people and people with normal hearing ability. Although innovations in sign language translation technology aim to tear down this communication barrier, the majority of existing sign language translation systems are either intrusive or constrained by resolution or ambient lighting conditions. Moreover, these existing systems can only perform single-sign ASL translation rather than sentence-level translation, making them much less useful in daily-life communication scenarios. In this work, we fill this critical gap by presenting DeepASL, a transformative deep learning-based sign language translation technology that enables ubiquitous and non-intrusive American Sign Language (ASL) translation at both word and sentence levels. DeepASL uses infrared light as its sensing mechanism to non-intrusively capture the ASL signs. It incorporates a novel hierarchical bidirectional deep recurrent neural network (HB-RNN) and a probabilistic framework based on Connectionist Temporal Classification (CTC) for word-level and sentence-level ASL translation respectively. To evaluate its performance, we have collected 7,306 samples from 11 participants, covering 56 commonly used ASL words and 100 ASL sentences. DeepASL achieves an average 94.5% word-level translation accuracy and an average 8.2% word error rate on translating unseen ASL sentences. Given its promising performance, we believe DeepASL represents a significant step towards breaking the communication barrier between deaf people and hearing majority, and thus has the significant potential to fundamentally change deaf people's lives.

==> ASL_CR - Copy/abstract.tex <==
%!TEX root = sensys2017.tex

%%
%In the U.S., there are over 28 million people considered deaf or hearing disabled.
%Although American Sign Language (ASL) is the predominant language used by deaf people, 
There is an undeniable communication barrier between deaf people and people with normal hearing ability.
%the Deaf community and people with normal hearing ability. 
%
Although innovations in sign language translation technology aim to tear down this communication barrier, the majority of existing sign language translation systems are either intrusive or constrained by resolution or ambient lighting conditions.
%
Moreover, these existing systems can only perform single-sign ASL translation rather than sentence-level translation, making them much less useful in daily-life communication scenarios.  
%
In this work, we fill this critical gap by presenting \textit{{\sysname}}, a transformative deep learning-based sign language translation technology that enables ubiquitous and non-intrusive American Sign Language (ASL) translation at both word and sentence levels.
%
{\sysname} uses infrared light as its sensing mechanism to non-intrusively capture the ASL signs.
%as an unobtrusive sensing mechanism to capture sign language.
%uses infrared light as its sensing mechanism
It incorporates a novel hierarchical bidirectional deep recurrent neural network (HB-RNN) and a probabilistic framework based on Connectionist Temporal Classification (CTC) for word-level and sentence-level ASL translation respectively. 
%a novel hierarchical bidirec-tional recurrent neural network (HB-RNN) model for ASL wordrecognition. The HB-RNN effectively combines the isolated ASLcharacterstics of both hands into an integrated representation forASL recognition at the word level. Second, DeepASL incorporates aprobabilistic framework based on Connectionist Temporal Classifica-tion (CTC) that captures probabilistic dependencies between wordscontained in one complete sentence. This eliminates the restrictionof segmenting the whole sentence into individual words, and thusenables translating the whole sentence end-to-end directl
%
%To examine the performance of {\sysname}, we have collected $3632$ samples from $11$ participants, covering $25$ most commonly used ASL words and $100$ ASL sentences.
%
To evaluate its performance, we have collected $7,306$ samples from $11$ participants, covering $56$ commonly used ASL words and $100$ ASL sentences.
%
{\sysname} achieves an average $94.5\%$ word-level translation accuracy and an average $8.2\%$ word error rate on translating unseen ASL sentences.
%To demonstrate the resilience of {\sysname} to 
%We have also collected 1178 samples to examine the resilience of {\sysname} to different usage scenarios. 
%
%{\sysname} achieves a $91.8\%$ word-level recognition accuracy in the worst-case scenario, demonstrating its great robustness.
%
%Given its promising performance, we believe {\sysname} could revolutionize the prospects of millions of deaf people, helping them break the communication barrier and naturally communicate with others in everyday life.
Given its promising performance, we believe {\sysname} represents a significant step towards breaking the communication barrier between deaf people and hearing majority, and thus has the significant potential to fundamentally change deaf people's lives.


%To achieve sentence-level ASL translation, we present an innovative approach that builds on top of the skeleton joints information of hands and arms extracted from infrared images, and combines the trajectories hierarchical bidirectional Long Short-Term Memory recurrent neural network (HB-LSTM RNN) and Connectionist Temporal Classification (CTC), trained entirely end-to-end without segmenting individual words within each sentence.
%To achieve sentence-level ASL translation, we present an innovative approach that builds sign language models by hierarchically combining the trajectories of skeleton joints of hands extracted from infrared images, trained using Connectionist Temporal Classification (CTC) loss function entirely end-to-end without segmenting individual words within each sentence.
%
%To achieve sentence-level ASL translation, we present an innovative approach that builds sign language models by hierarchically combining the trajectories of skeleton joints of hands extracted from infrared images, trained entirely end-to-end without segmenting individual words within each sentence.


%are not designed for daily usage in real-world settings

%system such as ASL often requires a synchronous language role model. It is our goal to develop an affordable and reliable ASL recognition system to provide instantaneous feedback to individuals learning ASL, such as parents and family members of children who are deaf, as well as the child who is deaf. Such a system has the potential to bypass the need for a language role model if it can provide sign accuracy feedback instantaneously

==> ASL_CR - Copy/ack.tex <==
%!TEX root = sensys2017.tex

% \section{Acknowledgement}
% \label{sec.ack}
%%
\noindent
%
We would like to thank Dr. John Stankovic for being the shepherd of this paper. 
%
We are also grateful to the anonymous SenSys reviewers for their valuable reviews and insightful comments. 
%
This research was partially funded by NSF awards \#1565604 and \#1617627.
%We thank our shepherd Dr. John Stankovic and the anonymous SenSys reviewers for their valuable reviews and insightful comments.
%We are grateful to Nvidia for their donation of GPU to support this work.
%We also thank the participants who helped collect our dataset.

==> ASL_CR - Copy/algorithm.tex <==
%!TEX root = sensys2017.tex

\section{System Details}
\label{sec.algorithm}


%%
\subsection{ASL Characteristics Extraction}
%
The skeleton joints data provided by the {\leap} sensor is noisy in its raw form. 
%It is necessary to filter out the noises before meaningful body movement information can be extracted from the CSI measurements.
%
As our first step, we apply a simple Savitzky-Golay filter~\cite{savitzky1964smoothing} to improve the signal to noise ratio of the raw skeleton joints data.
%
We select the Savitzky-Golay filter because of its effectiveness in smoothing skeleton joints data~\cite{Zhu2016,du2015hierarchical}.
%To improve the signal to noise ratio of the raw skeleton joints data, we apply a simple Savitzky-Golay filter~\cite{savitzky1964smoothing} to preprocess the raw data due to its effectiveness in smoothing skeleton joints data~\cite{Zhu2016,du2015hierarchical}.
%
Specifically, let $J_{i,j,t} = (x_{i,j,t}, y_{i,j,t}, z_{i,j,t}),~i = \{left, right\},~j = \{1, ..., N\},~t = \{1, ..., T\}$ denote the $t$-th frame of the temporal sequence of the 3D coordinates of the skeleton joints of fingers, palms and forearms of a single ASL sign, where $x$, $y$, $z$ denote the 3D coordinates of the skeleton joints, $i$ is the hand index, $j$ is the skeleton joint index (see Figure~\ref{fig:skeleton} for the skeleton joints tracked by the Leap Motion sensor), $t$ is the frame index, $N$ denotes the total number of skeleton joints in one hand, and $T$ denotes the total number of frames included in the temporal sequence.
%Let $J_{i,j,t} = (x_{i,j,t}, y_{i,j,t}, z_{i,j,t}),~i = left, right,~j = 1, ..., N,~t = 1, ..., T$ denote the temporal sequence of the 3D coordinates of the skeleton joints provided by {\leap}, where $i$ denotes the type of hand, $j$ indexes the skeleton joints, $t$ indexes the frame, $T$ is the total length of the sequence and $N$ is the number of skeleton joints. 
% In our implementation, we use the information of 28 skeleton joints of each hand ($N = 28$) and the length of sequences is a variable which depends on the duration and sampling rate of this sequence.  
%As the first step, we apply the Savitzky-Golay filter~\cite{savitzky1964smoothing} to the temporal sequence $J_{i,j,t}$ to remove the noise in the raw skeleton data.
%as it is commonly adopted by the state-of-the-art skeleton deep network works~\cite{du2015hierarchical, zhu2016co,song2016end}. 
%
The Savitzky-Golay filter is designed as
%
\begin{equation} 
\widetilde{J}_{i,j,t} = (-3J_{i,j,t-2} + 12J_{i,j,t-1} + 17J_{i,j,t} + 12J_{i,j,t+1} - 3J_{i,j,t+2})/35
\end{equation}
%
where $\widetilde{J}_{i,j,t}$ denotes the smoothed 3D coordinates of the skeleton joints in the $t$-th frame.

\vspace{-3mm}
\begin{figure}[h]
\centering
\includegraphics[scale=0.47]{Images/algorithm/skeleton.pdf}
\vspace{-2mm}
\caption{The skeleton joints tracked by the Leap Motion sensor.}
\vspace{-2mm}
\label{fig:skeleton}
\end{figure} 

% As pointed out in \S~\ref{primerASL}, a dynamic ASL is represented by three parts of core information: (1) spatial relationships among fingers and palm of either hand; (2) spatial relationship between two hands; (3) hand movement. Thus, in order to effectively learn comprehensive representations, modeling each of these parts and its combination is important. Therefore, we propose to extract two features of an ASL from raw data that are capable of representing this core information.

%
Based on the smoothed temporal sequence of the skeleton joints data, we extract the key characteristics of ASL signs including hand shape, hand movement and relative location of two hands from each frame of the sequence.
%Next, given that the performed ASL signs are independent of their absolute spatial 3D coordinates, we create a unified 3D coordinate system whose origin is at the palm center of the right hand and normalize the smoothed skeleton joints to this new coordinate system.
%Under this unified coordinate system, we extract the key characteristics of ASL signs including hand shape, hand movement and relative location of two hands from each frame of the temporal sequence.
%Specifically, since hand shape is independent of the location of the hand, we extract the hand shape information of both left and right hands by zero-centering the 3D coordinates of the skeleton joints on all the fingers related to the palm center of the right hand.
Specifically, since hand shape is independent of the absolute spatial location of the hand and is characterized by the relative distances among skeleton joints of palm and fingers, we extract hand shape information of both left and right hands by zero-centering the palm center of the right hand and then normalizing the 3D coordinates of the skeleton joints to it as
%
\begin{equation} 
S_{i,j,t} = \widetilde{J}_{i,j,t} - \widetilde{J}_{i,j = right\_palm\_center,t.}
\vspace{1.5mm}
\end{equation}
%where $S_{i,j,t}$ denotes the normalized skeleton joint coordinates of both hands. 
%As such, $S$ extracts the hand shape information of both hands. 
%Moreover, since right palm center is zero-centered, $S_{i=left}$ also extracts the relative location from left hand to right hand. 
%
By doing this, the information of the relative location of the left hand to the right hand is also encoded in $S_{i=left,j,t}$. 
%
Lastly, we extract hand movement information of both left and right hands as the spatial displacement of each skeleton joint between two consecutive frames defined as
% follows:
\begin{equation}
\vspace{-0.5mm}
  M_{i,j,t}=\begin{cases}
    (0, 0, 0), & \text{if $t = 1$} \\
    \widetilde{J}_{i,j,t} - \widetilde{J}_{i,j,t-1}, & \text{if $t = 2, ..., T$}.
      \end{cases}
  \vspace{1.5mm}
\end{equation}
%where $M_{i,j,t}$ denotes the spatial displacement vector of each skeleton joint in the $t$-th frame.

%%
Taken together, the ASL characteristics extracted from each frame of the temporal sequence of 3D coordinates of the skeleton joints result in four spatio-temporal ASL characteristics trajectories that capture information related to: 1) right hand shape, 2) right hand movement, 3) left hand shape (it also encodes the information of the relative location of the left hand to the right hand), and 4) left hand movement, respectively.
%
We denote them as $\bm{S}_{right}$, $\bm{M}_{right}$, $\bm{S}_{left}$, and $\bm{M}_{left}$ accordingly.
%
%Therefore, we confirm that hand shape, movement and relative location information is extracted. 
%In particular, this information consists of four trajectory sequences: 1) hand shape of right hand; 2) movement of right hand; 3) hand shape of left hand and relative location to the right hand; and 4) movement of left hand ($S_{right}$, $M_{right}$, $S_{left}$, $M_{left}$ respectively).


%\vspace{1mm}
%\noindent
%\textbf{Hand Shape and Relative Location Extraction:} 
%Hand shape is independent of the location of hands. 
%Thus we zero-center the right palm center (denoted as $right\_palm$), given as follows:
%\begin{equation} 
%S_{i,j,t} = \widetilde{J}_{i,j,t} - \widetilde{J}_{i,j = right\_palm,t}
%\end{equation}
%where $S_{i,j,t}$ denotes the normalized skeleton joint coordinates of both hands. 
%As such, $S$ extracts the hand shape information of both hands. 
%Moreover, since right palm center is zero-centered, $S_{i=left}$ also extracts the relative location from left hand to right hand. 
%For illustration purpose, we show the extracted hand shape and movement information of right middle finger tip joint for ``big'' and ``small'' in Figure~\ref{dia.keyinfo}. 
%The solid lines denote the temporal information of ``big'' while dashed lines denote ``small''. 
%As we can see, the hand shape and movement information of two signs begin to differentiate themselves at 0.3 seconds.  
% Specifically, y coordinate (perpendicular to chest, parallel to ground) information diverges the most (around 125 mm difference) due to the different position requirements of both ASL.

%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.33]{Images/algorithm/keyinfo.pdf}
%\caption{Illustration of hand shape and movement information of right middle finger tip joint for ``big'' and ``small''.}
%\vspace{-3mm}
%\label{dia.keyinfo}
%\end{figure} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
%\vspace{1mm}
%\noindent
%\textbf{Movement Extraction:}
%
%We then extract the movement information as spatial displacement of each joint between two consecutive frames, defined as follows:

%Figure~\ref{dia.keyinfo}(b) illustrates the extracted movement information. 
%As we can see, the movement along x direction (parallel to chest and ground) displays the largest difference starting from 0.6 seconds to 1.0 seconds. 
%This is because when performing ``big'' and ``small'', one is required to move her hands to different directions. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Word-Level ASL Translation}

%%
In this section, we first provide the background knowledge of bidirectional recurrent neural network (B-RNN) and Long Short-Term Memory (LSTM) to make the paper self-contained. 
%
We then describe our proposed hierarchical bidirectional deep recurrent neural network (HB-RNN) which is designed upon B-RNN and LSTM for single-sign word-level ASL translation. 
%
Finally, we describe the architectures of four comparative models that we use to validate the design choice of our proposed model.

%In this section, we provide details about the algorithm that solves word-level ASL recognition problem. 
%To put our model into context, we begin with the primer on recurrent neural network (RNN) and bidirectional Long-Short Term Memory (B-LSTM). 
%Next, we describe our hierarchical bidirectional LSTM model that incorporates both coordinate and trajectory information extracted from skeleton joints.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% 
\vspace{2mm}
\subsubsection{A Primer on Bidirectional RNN and LSTM}
~\newline
%
RNN is a powerful model for sequential data modeling~\cite{graves2012supervised}.
%have outperformed traditional techniques that model a temporal sequence. 
%
It has been widely used and has shown great success in many important tasks such as speech recognition~\cite{graves2013speech}, natural language processing~\cite{socher2011parsing}, language translation~\cite{sutskever2014sequence}, and video recognition~\cite{donahue2015long}.
%
Specifically, given an input temporal sequence $\textbf{x} = (x_{1}, x_{2}, ..., x_{T})$, where in our case $x_{t}$ is the $t$-th frame of the spatio-temporal ASL characteristics trajectories, the hidden states of a recurrent layer $\textbf{h} = (h_{1}, h_{2}, ..., h_{T})$ and the output $\textbf{y} = (y_{1}, y_{2}, ..., y_{T})$ of a RNN can be obtained as:
\begin{equation} 
\label{equ.rnn1}
h_{t} = \theta_{h} (W_{xh} x_{t} + W_{hh} h_{t-1} + b_{h})
\vspace{0.5mm}
\end{equation}
%
\begin{equation}
\label{equ.rnn2}
y_{t} =\theta_{y} (W_{ho} h_{t} + b_{o})
\vspace{0.5mm}
\end{equation}
where $W_{xh}$, $W_{hh}$, and $W_{ho}$ are connection weight matrices, $b_h$ and $b_o$ are bias values, and $\theta_h$ and  $\theta_y$ are activation functions.

\begin{figure}[b]
\centering
\includegraphics[scale=0.348]{Images/algorithm/B-LSTM.pdf}
\vspace{-2mm}
\caption{The network architecture of bidirectional RNN (B-RNN).}
\vspace{-2mm}
\label{fig:b-rnn}
\end{figure} 

%%
The RNN model described above only contains a single recurrent hidden layer and is unidirectional.
%
One limitation of the unidirectional RNN is that it could only look backward and thus can only access the past information at each time point in the temporal sequence for inference.
%to infer the sign being performed. 
%
In the context of sign language translation, this limitation could cause translation errors when different signs share very similar characteristics at the beginning of the signs. 
%
To address this limitation, we propose to use bidirectional RNN (B-RNN)~\cite{schuster1997bidirectional} as the building block in our design. 
%
Figure~\ref{fig:b-rnn} illustrates the network architecture of a B-RNN.
%
As shown, B-RNN has two separate recurrent hidden layers, with one pointing backward (i.e., backward layer) and the other pointing forward (i.e., forward layer).
%
As such, a B-RNN can look both backward and forward, and can thus utilize both the past and future information at each time point in the temporal sequence to infer the sign being performed.

%We choose RNNs with the LSTM architecture because they can efficiently capture the temporal patterns in the temporal sequences of an ASL sign~\cite{hochreiter2001gradient}. 
%However, many ASL signs share very similar starting movement. 
%This could cause translation errors when different ASL signs share very similar characteristics at the beginning of the signs.
%In contrast, the bidirectional architecture can look backward and forward, and thus can access both the past and future information at each time point in the temporal sequence.
%By leveraging the recurrent structure of RNN, each time point in the sequence is able to learn to use the past information. 
%As such, a unidirectional RNN is capable of making meaningful prediction by associating the current and past information. 
%Moreover, one might start to perform from a hand resting point or transitioning from the same previous ASL word. 
%To address this problem, we propose a bidirectional RNN (B-RNN) model which can access to both past and future information of a sequence at each time point~\cite{schuster1997bidirectional}. 
%As such, each time point is equipped with the global view of the entire sequence and thus is able to make more reasonable prediction. 
%Moreover, by aggregating all predictions of each time point into one global prediction, B-RNN tolerates the length variation problem of different sample sequences. 
%We choose B-RNN other than the traditional unidirectional RNN because the unidirectional architecture could only look backward and thus can only use the past information at each time point in the temporal sequence to infer the sign being performed. 


%%
The recurrent structure of RNN enables it to learn complex temporal dynamics in the temporal sequence. 
%
However, it can be difficult to train a RNN to learn long-term dynamics due to the vanishing and exploding gradients problem~\cite{hochreiter2001gradient}.
%resulting from propagating the gradients down through the many layers of the recurrent network.
%due to vanishing and exploding gradient problem, 
%RNN typically have difficulties in handling long-term dependency among input temporal sequence. 
%
To solve this problem, Long Short-Term Memory (LSTM)~\cite{hochreiter1997long} was invented which enables the network to learn when to forget previous hidden states and when to update hidden states given new input.
%
This mechanism makes LSTM very efficient at capturing the long-term dynamics. 
%Specifically, a LSTM cell contains an input gate $i_{t}$, a forget gate  $f_{t}$, an output gate $o_{t}$, a hidden state $h_{t}$, and an internal memory cell state $c_{t}$. 
%%
%In order to model the temporal dependencies of these four trajectories, we propose to use recurrent neural networks (RNN) which leverages the contextual information. 
%
Given this advantage, we use B-RNN with LSTM architecture in our design to capture the complex temporal dynamics during signing.
%In our case, given that an ASL sequence can be quite long and thus incurs long-term time dependency, we use B-RNN with LSTM architecture for handling long-term dependency problem in ASL sequence. 

%vanilla RNN might not work well due to the gradient vanishing and exploding problem~\cite{hochreiter2001gradient}. 
% 
%We do not show the formula of LSTM as we use the traditional LSTM proposed in~\cite{hochreiter1997long}.  


%
%In practice,
%given an input temporal sequence $\textbf{\textit{x}} = (x_{1}, x_{2}, ..., x_{T})$ and hidden states of recurrent layer $\textbf{\textit{h}} = (h_{1}, h_{2}, ..., h_{T})$, the output $\textbf{\textit{y}} = (y_{1}, y_{2}, ..., y_{T})$ 
%
%the output can be calculated as: 
 %\begin{equation} 
 %f_{t} = \sigma(W_{xf} x_{t} + W_{hf}h_{t-1} + b_{f})
 %\vspace{-0mm}
 %\end{equation}
 %
 %\begin{equation} 
 %i_{t} = \sigma(W_{xi} x_{t} + W_{hi} h_{t-1} + b_{i})
 %\vspace{-0mm}
 %\end{equation}
 %
 %\begin{equation} 
 %o_{t} = \sigma(W_{xo}x_{t} + W_{ho}h_{t-1} + b_{o})
 %\vspace{-0mm}
 %\end{equation}
 %
 %\begin{equation} 
 %c_{t} = f_{t} \odot c_{t-1} + i_{t} \odot tanh(W_{xc}x_{t} + W_{hc} h_{t-1} + b_{c})  
 %\vspace{-0mm}
 %\end{equation}
 %
 %\begin{equation} 
% h_{t} =o_{t} \odot tanh(c_{t})
 %\vspace{-0mm}
% \end{equation}
 %
% \begin{equation}
%  \label{equ.rnn2}
% y_{t} =\theta_{y} (W_{hy} h_{t} + b_{y})
% \end{equation}
%
%where all $W$ are connection weight matrices and all $b$ are biases, $\sigma(\cdot)$ is sigmoid function and $\odot$ is Hadamard product.

%%
% Specifically, to facilitate the modeling of long-term dependency,  a LSTM cell introduces an input gate $i_{t}$, a forget gate  $f_{t}$, an output gate $o_{t}$, a hidden state $h_{t}$, and an internal memory cell state $c_{t}$. In practice, given an input temporal sequence $\textbf{\textit{x}} = (x_{1}, x_{2}, ..., x_{T})$ and hidden states of recurrent layer $\textbf{\textit{h}} = (h_{1}, h_{2}, ..., h_{T})$, the output $\textbf{\textit{y}} = (y_{1}, y_{2}, ..., y_{T})$ can be calculated as: 


% Recently recurrent neural networks (RNN) have outperformed traditional techniques that model  a temporal sequence. Given an input temporal sequence $\textbf{\textit{x}} = (x_{1}, x_{2}, ..., x_{T})$ and hidden states of recurrent layer $\textbf{\textit{h}} = (h_{1}, h_{2}, ..., h_{T})$, the output $\textbf{\textit{y}} = (y_{1}, y_{2}, ..., y_{T})$ can be calculated as follows~\cite{graves2012supervised, graves2014towards, graves2013speech}:
%
% \begin{equation} 
% \label{equ.rnn1}
% h_{t} = \theta_{h} (W_{xh} x_{t} + W_{hh} h_{t-1} + b_{h})
% \vspace{-0mm}
% \end{equation}

% The recurrent structure of hidden states ensures the relay of memory and thus facilitates RNN of its modeling in temporal sequence. 

% However, due to vanishing and exploding gradient problem, RNN typically have difficulties in handling long-term dependency among input temporal sequence~\cite{hochreiter2001gradient}. To solve this problem, LSTM architecture is proposed which replaces the hidden layer of RNN with more complex recurrent units~\cite{hochreiter1997long}. Figure \ref{dia.LSTM} illustrates a single recurrent unit of LSTM. Specifically, a LSTM recurrent unit contains an input gate $i_{t}$, a forget gate  $f_{t}$, an output gate  $o_{t}$, a hidden state  $h_{t}$, and an internal memory cell state  $c_{t}$. The activation of three gates and two states are given as follows:


% In order to leverage the \textit{contextual information} of both past and future of a frame in the temporal sequence, bidirectional recurrent neural network (BRNN) architecture was proposed~\cite{schuster1997bidirectional}. As illustrated in the Figure~\ref{dia.BRNN}, BRNN contains forward and backward units in the hidden layer. By connecting the two units to the same output layer, BRNN is capable of incorporating the memory of both past and future frames. In our implementation, we use LSTM as the recurrent units in the hidden layer of BRNN, as bidirectional LSTM recurrent neural network (B-LSTM). 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
\centering
\includegraphics[scale=0.23]{Images/algorithm/HB_LSTM.pdf}
\caption{The architecture of the hierarchical bidirectional deep recurrent neural network (HB-RNN) for word-level ASL translation. For ASL signs that are performed using only one hand, only the corresponding half of the {\modelone} model is activated.}
\vspace{-2mm}
\label{dia.HB-RNN}
\end{figure}

%% 
\vspace{2mm}
\subsubsection{Hierarchical Bidirectional RNN for Single-Sign Modeling}
~\newline
%
Although four spatio-temporal ASL characteristics trajectories have been extracted from the raw skeleton joints data, they are isolated and at low level, and thus can not be directly used for word-level ASL translation.
%
Therefore, we propose a hierarchical model based on bidirectional deep recurrent neural network with the LSTM architecture (HB-RNN) to integrate the isolated low-level ASL characteristics into an organized high-level representation that can be used for word-level ASL translation.

%%
Figure~\ref{dia.HB-RNN} illustrates the architecture of the proposed HB-RNN model. 
%
At a high level, our HB-RNN model takes the four spatio-temporal ASL characteristics trajectories as its input, extracts the spatial structure and the temporal dynamics within the trajectories, and combines them in a hierarchical manner to generate an integrated high-level representation of a single ASL sign for word-level ASL translation.
%
As shown, our {\modelone} model consists of seven layers including three B-RNN layers ($bl_{1,2,3}$), two fusion layers ($fl_{1,2}$), one fully connected layer ($fc$), and one softmax layer ($sm$). 
%
Each of these layers has different structure and thus plays different role in the whole model.
%
Specifically, in the $bl_{1}$ layer, the four spatio-temporal ASL characteristics trajectories that capture information related to the right hand shape ($\bm{S}_{right}$), right hand movement ($\bm{M}_{right}$), left hand shape ($\bm{S}_{left}$), and left hand movement ($\bm{M}_{left}$) are fed into four separate B-RNNs.
%In the input layer, {\modelone} takes in four trajectories, which are fed into corresponding B-RNN, outputting forward and backward (f/b) sequences in $bl_{1}$.
%
These B-RNNs capture the spatial structure among skeleton joints and transform the low-level ASL characteristics into new representations of right hand shape, right hand movement, left hand shape, and left hand movement in both forward layer $\overrightarrow{h}$ and backward layer $\overleftarrow{h}$.
%
%In the first fusion layer $fl_{1}$, we concatenate the new representations of right (left) hand shape and right (left) hand movement together to obtain an integrated representation of the right (left) hand as follows
In the fusion layer $fl_{1}$, we concatenate the newly generated representations of right (left) hand shape and right (left) hand movement together as 
%$\lbrace\overrightarrow{h}_{bl_{1}}^{t}(S_{i}),\overleftarrow{h}_{bl_{1}}^{t}(S_{i}),\overrightarrow{h}_{bl_{1}}^{t}(M_{i}),\overleftarrow{h}_{bl_{1}}^{t}(M_{i}) \rbrace,~~i=right,left$, and feed the two concatenations into two B-RNNs in the $bl_{2}$ layer separately to obtain an integrated representation of the right (left) hand.
%
%\begin{equation} 
%\label{equ.concat}
$R_{bl_{1}}^{i,t} = \lbrace\overrightarrow{h}_{bl_{1}}^{t}(\bm{S}^{t}_{i}),\overleftarrow{h}_{bl_{1}}^{t}(\bm{S}^{t}_{i}),\overrightarrow{h}_{bl_{1}}^{t}(\bm{M}^{t}_{i}),\overleftarrow{h}_{bl_{1}}^{t}(\bm{M}^{t}_{i}) \rbrace,~~i=\{right,left\},$
%\end{equation}
and feed the two concatenations into two B-RNNs in the $bl_{2}$ layer separately to obtain an integrated representation of the right (left) hand.
%where $R^{fl_{1}}_{i,t}$ is concatenated representation of layer $fl_{1}$, and the $\overrightarrow{\textit{h}}$ and $\overleftarrow{\textit{h}}$ denote f/b activation, respectively. 
%We denote them as $\overrightarrow{\textit{h}}(S)_{i,t}$, $\overleftarrow{\textit{h}}()_{i,t}$, $\overrightarrow{\textit{h}}(M)_{i,t}$ and $\overleftarrow{\textit{h}}(T)_{i,t}$, where 
% Next, in the fusion layer $fl_{1}$, we concatenate all four inputs, given as follows: 
% where $R^{fl_{1}}_{i,t}$ is concatenated representation at frame $t$ of layer $fl_{1}$ . 
%In the first fusion layer $fl_{1}$, the finger gestures of the right hand and right hand movement characteristics are combined to obtain an integrated representation of the right hand while the finger gestures of the left hand and left hand movement characteristics are combined to obtain an integrated representation of the left hand.
%
Similarly, the two newly generated right and left hand representations are further concatenated together in the fusion layer $fl_{2}$ denoted as $R_{bl_{2}}^{t}$.
%
This concatenation is then fed into the B-RNN in the $bl_{3}$ layer to obtain a high-level representation in both forward layer and backward layer (denoted as $\overrightarrow{h}_{bl_{3}}^{t}(R^{t}_{bl_{2}})$ and $\overleftarrow{h}_{bl_{3}}^{t}(R^{t}_{bl_{2}})$) that integrates all the ASL characteristics of a single sign.  
%Similar to the $bl_{1}$ layer, these two newly obtained right and left hand representations are fed into another two separate B-RNNs in the $bl_{2}$ layer, and the representations generated by these two B-RNNs are further combined in the second fusion layer $fl_{2}$ to . 
%
Finally, we connect $\overrightarrow{h}_{bl_{3}}^{t}(R^{t}_{bl_{2}})$ and $\overleftarrow{h}_{bl_{3}}^{t}(R^{t}_{bl_{2}})$ to the fully connected layer $fc$.
%
The output of $fc$ is summed up across all the frames in the temporal sequence and then normalized by the softmax function in the softmax layer $sm$ to calculate the predicted word class probability given a sequence $J$:
 \begin{equation} 
\label{equ.sum}
O =  \sum\limits_{t=1}^T O_{fc}^{t}
\vspace{-1.2mm}
\end{equation}
%
\vspace{-0.4mm}
\begin{equation} 
\label{equ.sm}
p(C_{k} | J) =  \frac{e^{O_{k}}}{\sum\nolimits_{n=1}^{C}e^{O_{n}}}, k = 1, ..., C
\vspace{1.5mm}
\end{equation}
where $C$ denotes the total number of ASL words in the dictionary.
%, and $k$ is the ASL word class index. 
%Moreover, the logits at frame $t$ ($L_{t}$) encompass the contextual information from both past and future trajectory information and thus equipped with a global view of the entire trajectory. 
%
By accumulating results and normalizing across all the frames, our model is able to make inference based on the information of the entire sequence.
%
More importantly, it allows our model to handle ASL signs that have different sequence lengths as well as sequence length variation caused by signing speed.

%The temporal dynamics of the high-level representation is further modeled by another RNN in layer R3. 
%Finally, after the temporal patterns are extracted from the high-level representation, a fully connected layer FC and a softmax layer SL are used to classify the sign.




%Next similar to Equation~\ref{equ.concat}, we concatenate the output of $fl_{2}$ and get the high-level representation, denoted as $R^{fl_{2}}$. 
%After a final B-RNN layer $bl_{3}$, we feed both f/b activation (denoted as $\overrightarrow{\textit{h}}(R^{fl_{2}})_{t}$ and $\overleftarrow{\textit{h}}(R^{fl_{2}})_{t}$) to a fully connected layer $fc$, as the connection weight matrices are shared across time. It is derived as follows:   
%\begin{equation} 
%L_{t} =  W_{\overrightarrow{h}(R^{fl_{2}})_{}}\overrightarrow{\textit{h}}(R^{fl_{2}})_{t} + 
%             W_{\overleftarrow{h}(R^{fl_{2}})_{}}\overleftarrow{h}(R^{fl_{2}})_{t}
%\end{equation}
%where $W_{\overrightarrow{h}(R^{fl_{2}})_{}}$ and $W_{\overleftarrow{h}(R^{fl_{2}})_{}}$ are the connection weight matrices from layer $bl_{3}$ to layer $fc$, and $L_{t}$ denotes the logits of each frame $t$. At last, $L_{t}$ are summed up across time and normalized in softmax layer $sm$:
%
%Finally, the objective of {\modelone} is to minimize the cross-entropy between $p(k)$ and one-hot encoded ground truth vector $g(k)$, given as follows:
%
%\begin{equation} 
%Loss = -\frac{1}{C}\sum\limits_{k=1}^{C}g(k) ln (p(k))
%\vspace{-0.8mm}
%\end{equation}



%Our hierarchical model is inspired by \cite{du2015hierarchical}. However, in contrast to their idea of decomposing skeleton joints spatial parts, we propose to decompose into \textit{characteristics of ASL} to learn from the low-level representation effectively. 

%Specifically, outputs in $fl_1$, $R^{fl_{1}}_{right}$ and $R^{fl_{1}}_{left}$ are able to learn the right and left hand representation from low-level representation separately. 
%Intuitively, one element of $R^{fl_{1}}_{right}$ might represent the movement speed of right thumb finger (learned from movement trajectory); and one of  $R^{fl_{1}}_{left}$ might represent the included angle between the two fingers (learned from hand shape trajectory). 
%Next, by hierarchically combining right and left hand representation, $R^{fl_{2}}_{}$ learns a high-level representation that combines both hands. 
%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% 
\vspace{2mm}
\subsubsection{Comparative Models}
~\newline
%
To validate the design choice of our proposed HB-RNN model, we construct four comparative models as follows:

%To precisely capture the core information of ASL, our model includes four key components: (1) hand shape extraction; (2) movement extraction; (3) hierarchical structure of deep network; and (4) bidirectional structural RNN. 
%To validate our model choice, we construct four comparative baseline models, each missing one of the four key components:
\squishlist{
\item{
%
\textbf{HB-RNN-M:} a hierarchical bidirectional RNN model with hand movement information only. We compare this model with HB-RNN to prove the importance of the hand shape information.
} 
%
\item{
%
\textbf{HB-RNN-S:} a hierarchical bidirectional RNN model with hand shape information only. We compare this model with HB-RNN to prove the importance of the hand movement information.
}

\item{\textbf{SB-RNN:} a simple bidirectional RNN model without hierarchical structure. We compare this model with HB-RNN to prove the importance of the hierarchical structure.
}
\item{\textbf{H-RNN:} a hierarchical unidirectional RNN model with forward recurrent layer only. We compare this model with HB-RNN to prove the significance of the bidirectional connection.
}
}\squishend

%%
The parameters of the proposed HB-RNN model as well as the four comparative models are listed in Table~\ref{tab.parameters}. 

\begin{table}[h]
\centering
\scalebox{0.82}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Category}                                                                    & \textbf{Model} & \textbf{RNN Layer 1}                  & \textbf{RNN Layer 2}                 & \textbf{RNN Layer 3}                 \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}One-Hand\\ ASL\\ Words\end{tabular}}  & HB-RNN-M              & 2 $\times$ 1 $\times$ 128  & -                        & -                        \\ \cline{2-5} 
                                                                            & HB-RNN-S              & 2 $\times$ 1 $\times$ 128  & -                        & -                        \\ \cline{2-5} 
                                                                            & SB-RNN                 & 2 $\times$ 1 $\times$ 128 & -                        & -                        \\ \cline{2-5} 
                                                                            & H-RNN                 & 1 $\times$ 2 $\times$ 64  & 1 $\times$ 1 $\times$ 128 & -                        \\ \cline{2-5} 
                                                                            & {\modelone}          & 2 $\times$ 2 $\times$ 32  & 2 $\times$ 1 $\times$ 64 & -                        \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Two-Hand\\ ASL\\ Words\end{tabular}} & HB-RNN-M              & 2 $\times$ 2 $\times$ 64  & 2 $\times$ 1 $\times$ 128 & -                        \\ \cline{2-5} 
                                                                            & HB-RNN-S              & 2 $\times$ 2 $\times$ 64  & 2 $\times$ 1 $\times$ 128 & -                        \\ \cline{2-5} 
                                                                            & SB-RNN                 & 2 $\times$ 1 $\times$ 256 & -                        & -                        \\ \cline{2-5} 
                                                                            & H-RNN                 & 1 $\times$ 4 $\times$ 64  & 1 $\times$ 2 $\times$ 64 & 1 $\times$ 1 $\times$ 128 \\ \cline{2-5} 
                                                                            &{\modelone}          & 2 $\times$ 4 $\times$ 32  & 2 $\times$ 2 $\times$ 32 & 2 $\times$ 1 $\times$ 64 \\ \hline
%Sentence                                                                    &\textbf{{\modeltwo}}          & 2 $\times$ 4 $\times$ 32    & 2 $\times$ 2 $\times$ 64   & 2 $\times$ 1 $\times$ 128  \\ \hline
\end{tabular}
}
\vspace{2mm}
 \caption{The parameters of our proposed HB-RNN model and the four comparative models. The parameters follow the format of 1 (unidirectional) or 2 (bidirectional) $\times$  \#RNNs $\times$ \#hidden units. 
 }
 \vspace{-7mm}
 \label{tab.parameters}
\end{table}

%For example, the dimension of the parameters of two hand {\modelone} in layer $bl_{1}$ is ordered as 2 (forward + backward RNN) $\times$ 4 (sets of bidirectional RNN) $\times$ 32 (number of hidden units).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%
\subsection{Sentence-Level ASL Translation}
\label{sec.algorithm2}
%%
In daily-life communication, a deaf person does not sign a single word but a complete sentence at a time.
%
Although the {\modelone} model described in the previous section is capable of transforming the low-level ASL characteristics into a high-level representation for word-level translation, when translating a complete ASL sentence, {\modelone} still requires pre-segmenting the whole sentence into individual words and then connecting every translated word into a sentence in the post-processing. 
%
This is not only complicated but also requires users to pause between adjacent signs when signing one sentence, which is not practical in daily-life communication. 

%%
To address this problem, we propose a probabilistic approach based on Connectionist Temporal Classification (CTC)~\cite{graves2006connectionist} for sentence-level ASL translation.
%that captures the probabilistic dependencies between words within one complete sentence
%\biyi {T2} 
%
CTC is the key technique that drives the modern automatic speech recognition systems such as Apple Siri and Amazon Alexa~\cite{mcgraw2016personalized}.
%
It eliminates the necessity of word pre-segmentation and post-processing, allowing end-to-end translation of a whole sentence.
%allowing modern speech recognition systems to use the whole sentences directly for building sentence-level speech recognition models.
%
Inspired by its success on sentence-level speech recognition, we propose a CTC-based approach that can be easily built on top of the {\modelone} model described in the previous section for sentence-level ASL translation.
%This approach eliminates the necessity of segmentation and postprocessing, allowing end-to-end translation of the whole sentence. 
%
Specifically, to realize sentence-level ASL translation based on CTC, we make the following modifications on {\modelone}:
%Specifically, we make the following modifications on top of {\modelone}:
%
%To implement CTC on learned representation, we make three modifications on {\modelone}:
\squishlist{
\item{
%We change original class labels. 
Let $V$ denote the ASL word vocabulary.
%We add a ``blank'' class into $V$, (i.e., $V'= V\cup\{blank\}$). 
%
We add a blank symbol $\{blank\}$ into the ASL word vocabulary: $V'= V\cup\{blank\}$.
%which essentially enables us to model the transition from one ASL word to another within a single sentence.
%
Essentially, this blank symbol enables us to model the transition from one word to another within a single sentence. 
}
\item{
We increase the capacity of the RNN layers (i.e., $bl_1$, $bl_2$ and $bl_3$) in HB-RNN to 2 $\times$ 4 $\times$ 32, 2 $\times$ 2 $\times$ 64, and 2 $\times$ 1 $\times$ 128, respectively (see Table \ref{tab.parameters} for the format definition). 
%The number of parameters is roughly twice as many as {\modelone} for two-hand ASL word recognition. 
This is because ASL sentences are more complex than ASL words and thus require more parameters for modeling.
}
\item{
%
%Since the label of sentence-level sequence no longer consists only one single sign, we cannot summarize all outputs over time and apply softmax consequently (Equation~\ref{equ.sum} and \ref{equ.sm}). 
%Instead, we separately apply softmax on the output of fully connected layer ($fc$) at each time step, generating a sequence of distributions of each class in $V'$.
%Since an ASL sentence consists of multiple signs, we replace the softmax layer in HB-RNN which computes the probability of a single sign with a new softmax layer which computes the probability of each class in $V'$ at each frame of the sequence.
Since an ASL sentence consists of multiple signs, we replace the softmax layer in HB-RNN which computes the probability of a single sign with a new softmax layer which computes the probabilities of a sequence of multiple signs.
% of a single sign with a new softmax layer which computes the probability of a sequence of multiple signs.
% time and hence making a global prediction, we change the $sm$ to a frame-wise softmax, given as:
%\begin{equation} 
%p(k)_{t} =  \frac{e^{L_{k,t}}}{\sum\nolimits_{k=1}^{C}e^{L_{k,t}}}
%\end{equation}
%where $L_{k,t}$ denotes the logit of $k^{th}$ class at frame $t$, $p(k)_{t}$ denotes the probability of $k^{th}$ class at frame $t$. 
%This change exposes frame-wise prediction of {\modelone}, enabling it to predict a sequence of ASL words.
%
}
\item{
%Given a model that outputs a sequence of discrete distributions over the token classes (vocabulary) augmented with a special ?blank? token, CTC computes the probability of a sequence by marginalising over all sequences that are defined as equivalent to this sequence. 
Based on the modified softmax layer, the probabilities of all the possible sentences formed by the word included in $V$ can be computed.
%
Given those probabilities, we compute the probability of a target label sequence by marginalizing over all the sequences that are defined as equivalent to this sequence. 
%
For example, the label sequence $'SL'$ is defined as equivalent to the label sequences $'SSL'$, $'SLL'$, $'S\underline{\hspace{2mm}} L'$ or $'SL\underline{\hspace{2mm}}'$, where $'\underline{\hspace{2mm}}'$ denotes the blank symbol $\{blank\}$. 
%
This process not only eliminates the need for word pre-segmentation and post-processing but also addresses variable-length sequences.
%Next, we take the log likelihood form of CTC probability as the loss function. By optimizing the loss function and updating parameters accordingly, {\modeltwo} is able to generate a labeling sequence iterating through each time step.
}
%We change the objective function. Given the sequence of distribution of classes in $V'$, CTC computes the probability of a target label sequence by marginalizing over all possible sequences that are defined as equivalent to this sequence. As a result, by using maximum likelihood estimation over the differentiable objective function, the ASL sentence recognition model ({\modeltwo}) can be trained end-to-end directly. 
%
\item{
Finally, we delete adjacent duplicate labels and remove all the blank symbols in the inferred label sequence to derive the translated sentence. 
%We do this by simply removing all blanks and repeated labels. 
%For example, $'SS\underline{\hspace{2mm}} L'$ or $'S\underline{\hspace{2mm}} LL\underline{\hspace{2mm}}'$ are decoded as $'SL'$.
}
}\squishend

%%
With all the above modifications, the end-to-end sentence-level ASL translation is achieved.
%During prediction, best path decoding or beam search decoding can be applied to determine label sequences. 











% % In this section, we provide details about the algorithm that solves sentence-level ASL recognition problem. We begin with a primer on Connectionist Temporal Classification, a key component that removes the necessity of sequence labeling alignment. For sentence-level ASL recognition, we then present {\modeltwo} which essentially appends one layer to the softmax layer of {\modelone} with Connectionist Temporal Classification loss (CTC).

% \subsection{A Primer on Connectionist Temporal Classification}
% Associated with RNN, the Connectionist Temporal Classification loss (CTC) is widely used in modern applications such as natural language processing and handwritten character recognition as it \textit{eliminates the effort of segmentation} of sequence data~\cite{graves2006connectionist}. In other words, without CTC traditional RNN can only be trained to make a series of independent classifications (given the input). As such, we have to pre-segment the sequence data to make sure that the labels align with data; and output needs extra post-processing to generate the final label sequence. At a high level, CTC regards the output of RNN (after softmax layer) as a probability distribution over all possible label sequences, given the input sequence of the RNN. Given this distribution, a differentiable loss function can be derived that maximizes the probability of the ground truth label sequence. 
% %More specifically, let $\Omega$ denotes the set of all possible classes of the training sequences, CTC constructs a new set $\Omega^\prime = \Omega\cup\lbrace$\textvisiblespace$\rbrace$, where \textvisiblespace denotes CTC blank symbol. 
% Therefore, during training process, end-to-end training can be achieved by using maximum likelihood and backpropagation algorithm. During prediction process, best path decoding or beam search decoding can be applied to determine label sequences. CTC can simultaneously remove the necessity of \textit{pre-segmentation} and solve the \textit{variable-length sequence} problem. 

% In our sentence-level ASL recognition problem, we have the inputs of a free-flow ASL sentence, performed by hands; and through some algorithm we hope to find a sequence of labels that \textit{translates} this sentence into speech. Meanwhile, recall that in layer $fc$, {\modelone} is capable of learning representations of ASL and outputting the logits over all possible labels $L_{t}$. By applying a softmax operation on $L_{t},~t=1, ...,T$, one could easily obtain a time series of probability distribution, which equals to all possible label sequences. It then can be converted to a CTC problem.

% \subsection{{\modeltwo} Architecture}
% \subsubsection{Hierarchical Bidirectional LSTM with CTC}
% To structure our model {\modeltwo}, we do two changes to {\modelone}: (1) change the softmax layer $sm$ to frame-wise softmax; and (2) replace the cross-entropy loss to CTC. In detail, Equation~\ref{equ.sum} of softmax layer $fc$ is changed to:
% %




 








==> ASL_CR - Copy/applications.tex <==
%!TEX root = sensys2017.tex


\section{Applications}

%%
The design of {\sysname} enables a wide range of applications. 
%
To demonstrate the practical value of {\sysname}, we have developed two prototype applications based on {\sysname}.
%
In this section, we briefly describe these two prototype applications.

%We have implemented two applications to demonstrate two usage scenarios of {\sysname}.



%In this section, we briefly describe how {\sysname} is implemented on these platforms. 
%We report the performance of {\sysname} on the three platforms in the next section.

%\subsection{Data Fetching and Preprocessing}
%{\sysname} automatically compress and record the {\leap} raw data in a binary file encoded by Python (Version 3.5.2) Numpy library (Version 1.12.1). This  file {\sysname} is then loaded into memory for preprocessing. We then use Numpy to implement Savizky-Golay smoothing filter, coordinate normalization and trajectory extraction. Due to the fact that Numpy uses C/C++ as low level computation, the runtime of data fetching and preprocessing is extremely low. 

%\vspace{0.5mm}
%\noindent
%\textbf{ASL Word Recognition:} We use Tensorflow (Version 1.0.1) \cite{tensorflow2015-whitepaper} to implement training and prediction of both one hand and two hand ASL word recognition of {\sysname}. The hyperparamters of {\modelone} is summarized in Table~\ref{tab.parameters}. We determine these parameters via cross-validation. No dropout is implemented, because we find no major difference is made after dropout is implemented. We initialize all connection weight matrices with random samples from truncated normal distribution with a standard deviation of 0.01. For each training step, we use back-propagation through time (BPTT) algorithm~\cite{werbos1990backpropagation} to get the derivatives of our loss function and then pass them with respect to each elements in connection weigth matrices. The model is trained using Adam optimizer \cite{kingma2014adam} with settings of a learning rate of $10^{-3}$, a first-moment momentum coefficient of 0.9, a first-moment momentum coefficient of 0.999 and a numerical stability of  $10^{-8}$. In each training step, mini-batches of size 32 is fed into {\modelone}. During prediction, we label the input as the class with highest probability.

%\vspace{0.5mm}
%\noindent
%\textbf{ASL Sentence Recognition:} We use Tensorflow to implement the training and prediction of personal interpreter of {\sysname}. Hyperparameters of this model is shown in Table~\ref{tab.parameters}.. We increase the number of hidden units because it helps to obtain better performance. This is because sentence-level ASL recognition is more complex from the perspective of modeling than word--level recognition and therefore a network with more complexity is more capable of model sentence-level ASL. In contrast to the implementation of ASL dictionary we apply dropout after fusion layers and fully connected layer ($fl_{1}$, $fl_{2}$ and $fc$; dropout rate $p = 0.5$). By doing this, model overfitting is prevented. We then use maximum likelihood estimation~\cite{graves2006connectionist} and BPTT alogrithm to train {\modeltwo}. All the weights are updated using Adadelta optimizer~\cite{zeiler2012adadelta} with learning rate of 1, decay rate of 0.95 , numerical stability of $10^{-8}$. In each training step, our model is trained on a mini-batch of size 32. We note that despite that ASL sentence recognition model shares very similar structure of ASL word recognition model, it takes much longer to train the model. In detail, the training process of ASL word recognition takes approximately 200 steps to converge with total time of roughly 5 minutes on GTX 1080 GPU, but this process of ASL sentence takes up to 40000 steps with up to 40 hours on the same GPU. This is because the introduction of CTC component of deep network brings enormous complexity to the model, and thus grandly complicate the optimization space. During prediction, we use beam decoder to predict the most likely ASL sentences, with beam width of 100~\cite{graves2006connectionist}. 



\subsection{Application\#1: Personal Interpreter}

%%
\vspace{0.5mm}
\noindent
\textbf{Use Scenario:} 
%
For the first application, {\sysname} is used as a \textit{Personal Interpreter}.
%that aims to bridge the communication gap between a deaf person and people with normal hearing ability in daily-life communications.
%Imagine a deaf person meets a new friend in a coffee shop and he wants to introduce himself to her. It is possible for them to write down and exchange sentences on a paper or using smartphones, but this process is not only time consuming but also an unnatural way to communicate. 
%
With the help of an AR headset, \textit{Personal Interpreter} enables real-time two-way communications between a deaf person and peole who do not understand ASL.
%%to enable a deaf person to communicate with 
Specifically, on one hand, \textit{Personal Interpreter} uses speech recognition technology to translate spoken languages into digital texts, and then projects the digital texts to the AR screen for the deaf person to see; 
%
on the other hand, \textit{Personal Interpreter} uses ASL recognition technology to translate ASL performed by the deaf person into spoken languages for peole who do not understand ASL.
%digital texts, and then them through the speaker 
%(also projects to screen for verification purpose). 
%This two-way communication is translated in real time.

%%
\vspace{0.5mm}
\noindent
\textbf{Implementation:}
%
We implemented \textit{Personal Interpreter} as a Microsoft Hololens application. 
%
Since Mircrosoft Hololens currently does not support hosting USB clients, we could not implement DeepASL in Mircrosoft Hololens.
%
Instead, we transmitted the ASL recognition results to Hololens via TCP/IP.
%
Figure~\ref{dia.holo} illustrates the usage scenario and a screenshot from AR perspective. 
%
As shown, the recognized ASL sentence is displayed in the green dialogue box in the Hololens application. 
%
%\biyi {T3} 
%
The tablet-AR set is burdensome to the deaf people, but we envision that in the future, the AR headset will be miniaturized and hence is much less burdensome for people to wear on a daily basis. 
%
Meanwhile, the future AR headset will be able to host a USB device, enabling direct data transmission from {\leap} to itself.


%Note that the operating system of Hololens cannot host a USB device, we enable data transmission from {\leap} to AR via TCP/IP. Once skeleton data is transmitted to tablet (or other host machines), it then transfers the recognized sentence to AR, which visualizes this sentence in a green dialogue box. 

%In addition, we design a AR software that implemented on Microsoft Hololens~\cite{hololens}, data stream is fed by a host machine via TCP/IP. 


\begin{figure}[h]
\centering
\includegraphics[scale=0.2]{Images/impl/ar.pdf}
\caption{The \textit{Personal Interpreter} application: (a) a deaf person performing ASL while wearing a Microsoft Hololens AR headset; (b) a screenshot from AR perspective.}
\vspace{-2mm}
\label{dia.holo}
\end{figure} 


%%
%{\sysname} is designed for two usage scenarios, both aiming to solve dire need of deaf persons. 
%The ASL dictionary mode helps user to look up a unknown ASL words effortlessly; and personal interpreter that translates ASL sentence into speech in real time. 



%%
\subsection{Application\#2: ASL Dictionary}

\vspace{0.5mm}
\noindent
\textbf{Use Scenario:} 
%
For the second application, {\sysname} is used as an \textit{ASL Dictionary} to help a deaf person look up unknown ASL words.
%that aims to help a user who wants to learn ASL.
%In the second application, {\sysname} is used as a personal ASL tutor that aims to help a user who wants to learn ASL to look up any unknown ASL word.
%
%This application is specifically designed for deaf persons who wants to look up one target ASL word.
%
Spoken languages (e.g., English) allow one to easily look up an unknown word via indexing. 
%For example, one simply types in the word 'sign' in the web browser through word that starts with 's' in a dictionary. 
Unfortunately, this is not the case for ASL. 
%
Imagine a deaf child who wants to look up an ASL word that she remembers how to perform but forgets the meaning of it. 
%
Without the help of a person who understands ASL, there is not an easy way for her to look up the ASL word. 
%
This is because unlike spoken languages, ASL does not have a natural form to properly index each gesture. 
%
\textit{ASL Dictionary} solves this problem by taking the sign of the ASL word as input and displays the meaning of this ASL word in real time. 

\vspace{0.5mm}
\noindent
\textbf{Implementation:} 
%%
We implemented \textit{ASL Dictionary} as a Microsoft Surface tablet application.
%
Figure~\ref{dia.dict} illustrates the usage scenario and a screenshot of the tablet application.
% 
%the application is a web-based app which takes in the {\leap} output, visualizes to the user, recognizes this word and then projected the information onto the screen. 
%We enable this process by: (1) Javascript API of {\leap} to visualize hands; (2) Python with Tensorflow to recognize in the back-end.    


\begin{figure}[h]
\vspace{0.2mm}
\centering
\includegraphics[scale=0.18]{Images/impl/app_tablet.pdf}
\vspace{-2mm}
\caption{The \textit{ASL Dictionary} application: (a) a deaf person looking up an ASL word ``help''; (b) a screenshot of the tablet application.}
\vspace{-2mm}
\label{dia.dict}
\end{figure}












==> ASL_CR - Copy/background.tex <==
%!TEX root = sensys2017.tex

\section{Background, State-of-the-Art, and Design Choice}
\label{sec.background}
\vspace{-2mm}
\noindent
%%
%1. A primer on LM
%2. Compare LM with other sensing modalities
%3. Two use cases and selected ASL

%%
%In this section, we first provide background knowledge about the characteristics of ASL.
%Based on the characteristics of ASL, we explain our design considerations on selecting the most appropriate sensing modality to capture the sign language to support daily-life communication scenarios.

%%
\subsection{Characteristics of ASL}
%
ASL is a complete and complex language that mainly employs signs made by moving the hands~\cite{hoza2007s}.
%ASL has a vocabulary of more than 7000 individual signs.
%
Each individual sign is characterized by three key sources of information: 1) hand shape, 2) hand movement, and 3) relative location of two hands \cite{hoza2007s, liddell2003grammar}. 
%
It is the combination of these three key characteristics that encodes the meaning of each sign.
%
As an example, Figure~\ref{fig:asl-hand} illustrates how these three characteristics altogether encode the meaning of two ASL signs: ``small'' and ``big''. 
%
Specifically, to sign ``small'', one starts with holding both hands in front of her with fingers closed (i.e., hand shape), and then moves two hands towards each other (i.e., hand movement and relative location).
%
In comparison, to sign ``big'', one starts with extending the thumb and index fingers to form a slightly bent 'L' shape (i.e., hand shape), and then moves two hands away from each other (i.e., hand movement and relative location). 

%%
\begin{figure}[h]
\centering
\includegraphics[scale=0.171]{Images/background/hand/hand2.pdf}
\vspace{-1mm}
\caption{Illustration on how hand shape, hand movement, and relative location of two hands altogether encodes the meaning of two ASL signs: ``small'' and ``big''.}
\vspace{-2mm}
\label{fig:asl-hand}
\end{figure} 

%%
It is worthwhile to note that, for illustration purpose, we have selected two of the most distinctive ASL signs to explain the characteristics of ASL. 
%Also note that one-handed ASL words are characterized by first two out of three aspects and because of the similarity we do not show examples. 
%
In fact, there are many ASL signs that involve very subtle differences in the three key characteristics mentioned above. 
%
Moreover, in real-world scenarios, ASL signs can be expressed under various conditions such as bright vs. poor lighting conditions, walking vs. standing; and indoor vs. outdoor environments.
% making the task of ASL recognition even more difficult
It is the subtle differences and the real-world factors altogether that makes the task of ASL translation challenging. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\vspace{-3mm}
\subsection{State-of-the-Art ASL Translation Systems}
%\vspace{-1.5mm}

%%
Based on the sensing modality the system uses, existing ASL translation systems can be generally grouped into four categories: 1) wearable sensor-based, 2) Radio Frequency (RF)-based, 3) RGB camera-based, and 4) Kinect-based systems.
%Unfortunately, these sensing modalities fall short on one or more requirements mentioned above.
However, each of them has fundamental limitations that prevent it from being practically useful for translating ASL in daily life scenarios.
%
Specifically,
%
wearable sensor-based systems \cite{kim2008bi, kosmidou2009sign, li2010automatic, li2012sign, wu2015real, tubaiz2015glove, praveen2014sign, abhishek2016glove, kanwal2014assistive} use motion sensors (accelerometers, gyroscopes), EMG sensors, or bend sensors to capture the movements of hands, muscle activities, or bending of fingers to infer the performed signs.
%
However, wearable sensor-based systems require attaching sensors to a user's fingers, palms, and forearms.
%
This requirement makes them very intrusive and impractical for daily usage.
%
RF-based systems \cite{melgarejo2014leveraging} use wireless signals as a sensing mechanism to capture hand movements. 
%
Although this contactless sensing mechanism minimizes the intrusiveness to users, wireless signals have very limited resolutions to ``see'' the hands.
%RF-based approaches fail to capture finger gesture and hand location information, which is critical for recognizing sign languages.
%
RGB camera-based systems \cite{starner1998real, zafrulla2010novel, brashear2003using}, on the other hand, are capable of capturing rich information about hand shape and hand movement without instrumenting users. 
%However, they suffer from bad performance in poor lighting conditions and noisy backgrounds in real-world scenarios.
However, they fail to reliably capture those information in poor lighting conditions or generally uncontrolled backgrounds in real-world scenarios.
%
Moreover, the videos/images captured may be considered invasive to the privacy of the user and surrounding bystanders.
%
Finally, although Kinect-based systems overcome the lighting and privacy issues of the RGB camera-based systems by only capturing the skeleton information of the user body and limbs \cite{chai2013sign, chai2013visualcomm}, they do not have enough resolution to capture the hand shape information, which plays a critical role on decoding the sign language.

%%
%There are many sensing modalities having been explored in prior work.
%Prior sign language recognition systems have  primarily explored motion sensors, EMG, flex sensors, radio, and RGB cameras as sensing modalities.
%Unfortunately, these sensing modalities fall short on one or more requirements mentioned above.
%Specifically, motion sensors, EMG, or flex sensors require instrumenting fingers, palms, and forearms of users, making them intrusive and impractical for daily usage.
%A recent alternative is to use wireless radio signals as a sensing mechanism \cite{melgarejo2014leveraging}. 
%Although this contactless sensing mechanism minimizes the intrusiveness to users, wireless signals have limitations on capturing hand shape information.
%RGB cameras, on the other hand, are able to capture rich information of hand shapes and movements without heavily instrumenting users. 
%However, they are constrained by poor lighting conditions and breach privacy. 
%\biyi {T5} While Microsoft Kinect seems to capture the movement of hand and preserve privacy, one of the key drawbacks is its lack of resolution to capture finger gestures, which is more important than any other information of ASL recognition. 

%At the first glimpse, it seems that ASL can be easily captured by motion sensors or EMG sensor. Although these sensors are able to capture hand movements, they fail to capture hand shape information. 
%On the other hand, RGB camera seems to be a good choice but it does not work well in poor lighting conditions. 
%Depth sensor works in dimmed light but it has multi-device interference problem~\cite{sarbolandi2015kinect}, meaning that we cannot have more than one device in one room. 
%Radio frequency (RF) signal seems to capture both hand shape and movement, but physical information captured by RF signal (e.g., Channel State Information) are too course grained. 
%Embedded with motion sensors, sensors gloves can be misled when one is walking. Besides, the form factor might be intrusive for deaf people. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
\subsection{Design Choice}
%\label{comparison}
%%
%Considering the difficulties, \textit{the key for developing an ASL recognition system for daily-life communications is to identify a suitable sensing modality that can precisely and robustly capture hand shape, hand movement and relative location of two hands under various real-life scenarios}.
%; and to identify differentiable patterns from these three sources for each sign }.
%Therefore, to recognize ASL, we must first find a suitable sensing modality that can precisely capture those three informational aspects as well as be robust to different real life conditions.
%In addition, the sensing modality has to be \textit{non-intrusive}, with minimum instrumentation on users and preserving the privacy of users themselves and others.



%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.425]{Images/background/leap.pdf}
%\vspace{-1mm}
%\caption{(a) Skeleton joints tracked by {\leap}; (b) Effective range of {\leap}. }
%\vspace{-3mm}
%\label{dia.leap}
%\end{figure} 


%%
In the design of {\sysname}, we use {\leap} as our sensing modality to capture ASL signs~\cite{leapmotion}. 
%
{\leap} overcomes the fundamental limitations of existing technologies and is able to precisely capture the three key characteristics of ASL signs under real-world scenarios in a non-intrusive manner. 
%meets all the requirements mentioned above and we believe it is the most appropriate sensing modality for developing a wearable personal ASL recognition system for daily-life communications.  
%
Specifically, {\leap} uses infrared light as its sensing mechanism.
%
This not only enables it to capture the signs in a contactless manner but also makes it ``see'' the signs in poor lighting conditions.
%
Moreover, {\leap} is able to extract skeleton joints of the fingers, palms and forearms from the raw infrared images.
% to track the movements of fingers, hands and forearms.
%Moreover, {\leap} uses skeleton joints of the fingers, palms and forearms other than the raw infrared images to track the movements of fingers, hands and forearms.
%
This preserves the privacy of the user and bystanders, and more importantly, provides enough resolution to precisely capture hand shape as well as hand movements and locations.
%the three key characteristics of ASL.
%Leap focuses on finger gestures which are more important than anything else for sign language, since fingers are how deaf people describe most of their words.
As an example, Figure~\ref{fig:asl-leapmotion} illustrates how the ASL signs of two words ``small'' and ``big'' are precisely captured by the temporal sequence of skeleton joints of the fingers, palms and forearms. 
%
%Finally, {\leap} is small and lightweight in form factor, making it suitable as a wearable.
%Finally, {\leap} is small and lightweight in form factor, making it suitable to be integrated into many personal devices such as a wearable.
%When worn on the chest, its 150$^{\circ}$ detection range provided by the on-board wide-angle lenses is wide enough to capture signs performed in daily-life communication scenarios. 

%In our design, we use {\leap} as our sensing modality~\cite{leapapi}. 
%It meets all the requirements mentioned above and we believe it is the most appropriate sensing modality for developing a wearable personal ASL recognition system for daily-life communications.  
%Specifically, {\leap} uses infrared light as its sensing mechanism.
%This makes {\leap} able to ``see'' the signs in poor lighting or even dark conditions.
%Moreover, {\leap} uses skeleton joints on fingers, palms and forearms (Figure~\ref{dia.leap}(a)) other than raw infrared images to track hands and forearms.
%This preserves the privacy and more importantly, provides a robust way to precisely capture hand shape, hand movement and relative location of two hands.
%As an example, Figure~\ref{dia.track} illustrates how these three key aspects of ASL signs for word ``small'' and ``big'' are precisely captured by skeleton joints. 
%Finally, {\leap} is small and lightweight in form factor (80 x 30 x 11.35 mm; 45 g), making it suitable as a wearable device.
%When worn on chest, the 150$^{\circ}$ detection range provided by the on-board fisheye cameras (Figure~\ref{dia.leap}(b)) is wide enough to capture signs performed in daily-life communications. 

\vspace{-1mm}
\begin{figure}[h]
\centering
\includegraphics[scale=0.166]{Images/background/track/track2.pdf}
\vspace{-6.5mm}
\caption{The skeleton joints of two ASL signs: ``small'' and ``big''.}
\vspace{-1.5mm}
\label{fig:asl-leapmotion}
\end{figure} 

%Specifically, it uses three on-board infrared LEDs to emit invisible light, and two fish-eye angle infrared cameras to capture the reflection. 
%The captured infrared images (video stream) are then transmitted through USB to its host machine for skeleton joints extraction. 
%In fact, {\leap} is able to extract up to 300 frames of skeleton joints per second in real time, even on a relatively low-end CPU (e.g., Intel i3). 
%Thanks to two fish-eye angle cameras, in operation, the effective detection range of {leap} 80 cm (150$^{\circ}$ wide), as shown in Figure~\ref{dia.leap}.(a). 
%As shown in Figure~\ref{dia.leap}.(b), at each frame, {\leap} extracts skeletal information of five joints of four bones of each finger, and additional three joints of palm center, wrist and elbow, with average position error of 0.2 mm~\cite{weichert2013analysis}. 
%In total, the spatial coordinate of 27 joints are extracted (5 joints x 5 fingers + 3 additional - 1 thumb = 27). 



%%
%Figure~\ref{dia.track} shows the visualization of how three informational aspects of ASL word \textit{small} and \textit{big} are captured by {\leap}. In comparison to Figure~\ref{dia.hands}, we can see that both hand shape and movement of both hands are perfectly captured and featured with skeleton joints. 
%As such, we confirm that all three aspects can be precisely captured by {\leap}. 
%%
To sum up, Table~\ref{tab.comp} compares {\leap} with other sensing modalities used in existing sign language translation systems. 
%
As listed, {\leap} has shown its superiority over other sensing modalities on capturing the three key characteristics of ASL signs in a non-intrusive manner without the constraint of ambient lighting condition.
%
We leverage this superiority in the design of {\sysname}.

\begin{table}[h]	
\begin{center}
%\tabcolsep 5.8pt
%\tiny
%\small
\scalebox{0.71}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Sensing}    	& \textbf{Hand}         	& \textbf{Hand}                  & \textbf{Hand}        	& \textbf{Intrusive}    & \textbf{Lighting}     \\ 
\textbf{Modality}    	& \textbf{Shape}         	& \textbf{Movement}          & \textbf{Location}    & \textbf{}			& \textbf{Condition}  \\ \hline
Motion + EMG + Bend      	& Captured 		& Captured 			& No                          & Yes                        & Any                        \\ \hline
RF                   		& No      				& Captured 			& No 			& No 			& Any                        \\ \hline
RGB Camera           	& Captured                   	& Captured                        & Captured               & Yes                        & Constrained  		\\ \hline
Kinect                 	& No      				& Captured 			& Captured 		& No 			& Any                       \\ \hline
Leap Motion 		& Captured          		& Captured            		& Captured               & No                          & Any                         \\ \hline
\end{tabular}
 }
 \vspace{0.5mm}
\caption{Comparison of sensing modalities for ASL translation.}
%among sign language translation systems of different
%\label{tab:dataset}
\vspace{-7.5 mm}
\label{tab.comp}
\end{center}
\end{table}  









==> ASL_CR - Copy/challenges.tex <==
%!TEX root = sensys2017.tex


\section{Challenges and Our Solutions}
\label{sec.challenges}
%%
\noindent
%
Although {\leap} has shown its superiority over other sensing modalities on capturing key characteristics of ASL signs, there is a \textit{significant gap} between the raw skeleton joints data and the translated ASL.
%Although {\leap} has shown its superiority for capturing key information in sign language, there is still a \textit{significant gap} between the raw skeleton joints data provided by {\leap} and the recognized ASL. 
%
In this section, we describe the challenges on transforming the raw skeleton joints data into translated ASL at both word and sentence levels. 
%
We also explain how {\sysname} effectively addresses those challenges.

%%
%\vspace{1.5mm}
%\noindent
%\textbf{Challenge 0:} 
%{\leap} provides the access to both raw video stream and skeleton joints data to capture shape and movement of ASL. However, translation ASL words and sentences indeed needs real-time performance on resource-limited wearable devices. Therefore, we do not use raw video stream as our datainput because processing it potentially involves using convolutional neural networks (CNN) which is computational expensive and thus cannot achieve real time performance. Instead we use recurrent neural network (RNN) on top of skeleton joint data because it is computational efficient on CPU. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
\vspace{1.0mm}
\noindent
\textbf{ASL Characteristics Extraction:}
%
{\leap} is \textit{not} designed for ASL translation.
%
Although {\leap} captures the skeleton joints of the fingers, palms and forearms, the key information that characterizes ASL signs (i.e., hand shape, hand movement, and relative location of two hands) is still buried in the raw skeleton joints data.
%Although {\leap} provides the skeleton joints data, the key information that characterizes ASL (hand shape, hand movement and relative location of two hands) is still buried in this data. 
%It is necessary to extract those key ASL characteristics from the raw skeleton data before any meaningful models can be developed for ASL translation.
%
%To address this challenge, we leverage the domain knowledge of ASL to extract the key ASL characteristics from the raw skeleton joints data, and then develop models on top of the extracted ASL characteristics for ASL translation.
To address this challenge, we leverage domain knowledge of ASL to extract spatio-temporal trajectories of ASL characteristics from the sequence of skeleton joints during signing, and develop models upon the extracted ASL characteristics for ASL translation.
%into low-level representations by isolating these key information of ASL from raw data .  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
\vspace{1.0mm}
\noindent
\textbf{ASL Characteristics Organization:} 
%
The extracted ASL characteristics are isolated and unorganized, and thus can not be directly used for ASL translation. 
%
This problem is exacerbated when the number of ASL signs to be translated scales up.
%
To address this challenge, we propose a hierarchical model based on deep recurrent neural network (RNN) that effectively integrates the isolated low-level ASL characteristics into an organized high-level representation that can be used for ASL translation.  
%hierarchical bidirectional deep recurrent neural network (HB-RNN)
%model the spatial structure and temporal dynamics of human
%The key information has been extracted, but these low-level representations are isolated and unorganized. In other words, there is still a significant gap between low-level representation and the final recognition of ASL.
%To address this challenge, we propose to hierarchically structure the recurrent neuron networks (RNN) to effectively organize and transform this low-level representation into high-level representation and thus make precise recognition on ASL.   

% Challenge: ASL involves a complicated trajectory of one or two hands. How to effectively organize low-level representation derived from pre-processing results.
% Solution: Hierarchical modeling for high-level representation.


%we propose a deep learning-based hierarchical model for word-level single-sign ASL translation.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
\vspace{1.0mm}
\noindent
\textbf{Similarity between Different Signs:} 
%
Although each ASL sign is uniquely characterized by its ASL characteristics trajectories, many ASL signs share very similar characteristics at the beginning of their trajectories (see Figure~\ref{fig:similarity} as an example). 
%This could cause translation errors when different ASL signs share very similar characteristics at the beginning of the signs.
%Although each ASL sign is uniquely characterized by its trajectory of hand shapes and movements, there are many ASL signs that have very similar trajectory at the beginning (Figure~\ref{fig:similarity}). 
%Moreover, one might start to perform from a hand resting point or transitioning from the same previous ASL word. 
%
This similarity confuses traditional RNN which is based on a unidirectional architecture.
%
This is because the unidirectional architecture can only use the past information at each time point in the trajectory to infer the sign being performed.
%This similarity will confuse traditional RNN, which is based on the unidirectional architecture and thus only has access to past trajectory information.
%that it can only ?look? backward and thus can only use the past information at each time point in the temporal sequence to infer the sign being performed.
To address this challenge, we propose a bidirectional RNN model which performs inference at each point of the trajectory based on both past and future trajectory information. 
%can access both the past and future information at each time point in the temporal sequence
%
%With the global view of the entire trajectory, our bidirectional RNN model is able to make much more accurate ASL translation.
With the global view of the entire trajectory, our bidirectional RNN model is able to achieve better ASL translation performance. 

\begin{figure}[h]
\centering
\includegraphics[scale=0.318]{Images/challenges/similarity.pdf}
\vspace{-3mm}
\caption{Similarity between two ASL signs: ``want'' and ``what''.}
\vspace{-2mm}
\label{fig:similarity}
\end{figure} 

%Thanks to recurrent structure of RNN, each time point in the sequence can learn to use the past information. As such, unidirectional RNN is capable of making meaningful prediction by associating the current and past information. However, many ASL signs share very similar starting movement. Moreover, one might start to perform from a hand resting point or transitioning from the same previous ASL word. In this way, unidirectional RNN, with the access to only past information, makes unreliable predictions on these time points. To address this challenge, we use bidirectional RNN which grants the access to both past and future information of a sequence for each time point. As such, each time point is equipped with global view of the entire sequence and thus is able to make more reasonable prediction. Meanwhile by aggregating all predictions of each time point into one global prediction, bidirectional RNN tolerates the length variation problem of different sample sequences.

% Challenge: many ASL has very similar starting movements in the trajectory. To achieve more robust performance, one needs to have a global view at each point of the trajectory. 
% Solution: Bidirectional-LSTM
% Another benefit of Bidirectional-LSTM is that it tolerates length variation for single word.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
\vspace{1.0mm}
\noindent
\textbf{ASL Sentence Translation:}
%\textbf{Segmentation of Label Sequence of ASL sentences:} 
%
To translate ASL sentences, existing sign language translation technologies adopt a framework which requires pre-segmenting individual words within the sentence. % in the first place.
%segmentation of the label sequence is necessary. 
However, this framework restricts sign language translation technologies to translate one single sign at a time and thus requires users to pause between adjacent signs when signing one sentence.
%However, this process is cumbersome, time-consuming and thus impractical for the real world application. 
%
To address this challenge, we propose to adopt a framework based on Connectionist Temporal Classification (CTC) that computes the probability of the whole sentence directly, and therefore, removes the requirement of pre-segmentation.
%CTC computes the probability of a sequence by marginalising over all sequences that are defined as equivalent to this sequence. This simultaneously removes the need for alignments and addresses variable-length sequences.
%To address this challenge, we propose to adopt a framework based on Connectionist Temporal Classification (CTC) that removes the requirement of pre-segmentation and thus enables translating the whole sentence end-to-end directly.
%To address this challenge, we propose a probabilistic approach based on Connectionist Temporal Classification (CTC) that captures probabilistic dependencies between words contained in one complete sentence.
%This eliminates the restriction of segmenting the whole sentence into individual words, and thus enables translating the whole sentence end-to-end directly.

%eliminate the necessity of segmentation by applying Connectionist Temporal Classificaiton (CTC) onto the top of our high-level representation extracted in ASL word recognition. In addition, by eliminating the process of segmentation our model also tolerates the length variation problem of ASL sentences. 

%%
%
To the best of our knowledge, {\sysname} is the first ASL translation framework that addresses these challenges and achieves accurate ASL translation performance at word and sentence levels.






==> ASL_CR - Copy/conc.tex <==
%!TEX root = sensys2017.tex


\section{Conclusion}
\label{sec.con}
\noindent
%%
In this paper, we present the design, implementation and evaluation of {\sysname}, a transformative deep learning-based sign language translation technology that enables ubiquitous and non-intrusive ASL translation at both word and sentence levels.
%
%\biyi {T2} 
%
At the word level, {\sysname} achieves an average $94.5\%$ translation accuracy over 56 commonly used ASL words. 
%
At the sentence level, {\sysname} achieves an average $8.2\%$ word error rate on translating unseen ASL sentences and an average $16.1\%$ word error rate on translating ASL sentences performed by unseen users over 100 commonly used ASL sentences. 
%
%We also showed that {\sysname} is able to recognize sentences that are not included in the training dataset.
%
%We have also examined the resilience of 
%{\sysname} has also demonstrated its resilience to various factors in real-world settings.
%{\sysname} achieves more than $91.8\%$ word-level recognition accuracy in various ambient lighting conditions, body postures, and interference sources, demonstrating its great robustness in real-world settings.
%
Given the innovation solution it provides and its promising performance, we believe DeepASL has made a significant contribution to the advancement of ASL translation technology.
%Given its promising performance, we believe {\sysname} represents a significant step towards breaking the communication barrier between the deaf people and the hearing majority.




==> ASL_CR - Copy/discussion.tex <==
%!TEX root = sensys2017.tex

%\section{Discussion and Future Work}
\section{Discussion}
\label{sec.diss}

%%
%\noindent
%The experience of design and evaluation of {\sysname} provides us with insights on both the promises and limitations of XXX. 
%
%In this section, we briefly elaborate on those insights. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{1mm}

\noindent
\textbf{Impact on ASL Translation Technology:} 
%
{\sysname} represents the first ASL translation technology that enables ubiquitous and non-intrusive ASL translation at both word and sentence levels.
%{\sysname} represents the first ASL translation technology that is able to translate ASL at both word and sentence levels with accurate translation performance.
It demonstrates the superiority of using infrared light and skeleton joints information over other sensing modalities for capturing key characteristics of ASL signs.
%
It also demonstrates the capability of hierarchical bidirectional deep recurrent neural network for single-sign modeling as well as CTC for translating the whole sentence end-to-end without requiring users to pause between adjacent signs.
%
Given the innovation solution it provides and its promising performance, we believe {\sysname} has made a significant contribution to the advancement of ASL translation technology.
% under real-life scenarios in a non-intrusive manner.
%
%ASL translation. 
%
%With its promising performance, we envision that the functionality of {\sysname} could be integrated into future generations of wearables in the form of eye glasses, cloth buttons, or necklace.

%hope that {\sysname} could inspire researchers in sensor-enabled smart systems to work on 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{1mm}

\noindent
\textbf{Initiative on ASL Sign Data Crowdsourcing:} 
%Our work demonstrates the significant potential of {\sysname} for becoming the technology to bridge the communication gap between deaf people and people with normal hearing ability.
%
Despite months of efforts spent on data collection, our dataset still covers a small portion of the ASL vocabulary.
%
To make {\sysname} being able to translate as many words as in the ASL vocabulary and many more sentences that deaf people use in their daily-life communications, we have taken an initiative on ASL sign data crowdsourcing. 
%
We have made our data collection toolkit publicly available.
%We open sourcing four core parts of our project: (1) Experimental setup tutorial; (2) Data collection software; (3) Data visualization software; (4) DeepASL dataset (link: anonymous for now). 
%Given the prevalence of Leap Motion, 
%We encourage both deaf community and research community to contribute to this initiative. 
%We will keep working proactively on DeepASL with potential contributors in the future and 
%We hope this initiative could serve as a seed to draw attentions of people who want to turn this vision into reality.
%
We hope our initiative could serve as a seed to draw attentions from people who share the same vision as we have, and want to turn this vision into reality. 
%
We deeply believe that, with the crowdsourced efforts, ASL translation technology can be significantly advanced.
%
With that, we could ultimately turn the vision of tearing down the communication barrier between the deaf people and the hearing majority into reality.

%We deeply believe that, with crowdsourced efforts, we can collectively make a significant contribution to our society.

%It has the significant potential to fundamentally changing the way deaf people live, enablingmillions of deaf people to naturally and easily communicatewith others on a day-to-day basis


%With limited resources, it is impossible for could find an full-fledged solution to this important but challenging problem.
%Thus, we argue that data collection crowd sourcing is in dire need to enlarge the vocabulary coverage of DeepASL. 
%
%



%The results achieved indicates our sensing system and techniques are promising.
%However, fundamentally solving the ASL translation requires tons of data.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\vspace{1mm}
%\noindent
%\textbf{Opportunities for Improvement:} 
%
% 1. Hot-gesture detection to enable real-time translation.
% 2. Applying NLP techniques.
%
%There are a number of opportunities to make {\sysname} better.
%For example, similar to the ``hot-word'' mechanism used to activate Apple Siri or Amazon Echo, we need to design a ``hot-gesture'' detection mechanism to activate {\sysname} when needed.
%We can also apply natural language processing techniques to improve the performance of ASL recognition at sentence level.
%We leave them to future work.







==> ASL_CR - Copy/evaluation.tex <==
%!TEX root = sensys2017.tex


\section{Evaluation}
\label{sec.evaluation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Experimental Setup}
%%
\vspace{1mm}
\subsubsection{Dataset Design}
%
~\newline
%
To evaluate the translation performance of {\sysname} at both word and sentence levels as well as its robustness under real-world settings, we have designed and collected three datasets: 
%
1) ASL Words Dataset; 2) ASL Sentences Dataset; and 3) In-the-Field Dataset. 
%We describe the details of these three datasets.
 
\vspace{1mm}
\noindent
\textbf{ASL Words Dataset}: 
%
%We design the \textit{ASL Words} dataset by following two key design considerations:
%\squishlist{
% \item{Since it is nearly impossible for us to collect all ASL words, we target ASL words that are representative of each category of the ASL vocabulary. 
% }
% \item{Training deep neural network requires a large dataset which contains enough variation in terms of gesture execution. We aim to collect a dataset whose size is comparable to those of other state-of-the-art skeleton deep networks. 
% }
%}\squishend
%
Since it is impossible to collect all the words in the ASL vocabulary, we target ASL words that are representative of each category of the ASL vocabulary.
%
In particular, we have selected 56 ASL words from five word categories: pronoun, noun, verb, adjective and adverb.
%
Table~\ref{tab.aslwords} lists the selected 56 ASL words. 
%Based on the above design considerations, we have selected 25 ASL words from five groups of words: pronoun, noun, verb, adjective and adverb. 
%
These words are among the top 200 most commonly used words in ASL vocabulary. 
%
Among these 56 words, 29 are performed by two hands and the rest 27 are performed by one hand (right hand). 

\vspace{-1mm}
\begin{table}[h]
\centering
\scalebox{0.92}{
\begin{tabular}{|c|p{6.5cm}|}
\hline
\textbf{Category} & \hspace{25mm} \textbf{Words}                      \\ \hline
pronoun           & who, I, you, \underline{what}, we, my, your, other                       \\ \hline
noun              & \underline{time}, food, drink, mother, \underline{clothes}, \underline{box}, \underline{car}, \underline{bicycle}, \underline{book}, \underline{shoes}, \underline{year}, boy, \underline{church}, \underline{family}  \\ \hline
verb              & \underline{want}, \underline{dontwant}, like, \underline{help}, \underline{finish}, need, thankyou, \underline{meet}, \underline{live}, \underline{can}, come \\ \hline
adjective         & \underline{big}, \underline{small}, hot, \underline{cold}, blue, red, \underline{gray}, black, green, white, old, \underline{with}, \underline{without}, \underline{nice}, bad, \underline{sad}, \underline{many}, sorry, few         \\ \hline
adverb            & where, \underline{more}, please, \underline{but}                     \\ \hline
\end{tabular}
}
\vspace{2mm}
\caption{The ASL Words Dataset (two-hand words are underlined).}
\vspace{-7mm}
\label{tab.aslwords}
\end{table} 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
%% 
\vspace{1mm}
\noindent
\textbf{ASL Sentences Dataset}:
%Similar to the design of the ASL Words Dataset, since it is impossible to collect all the possible sentences, we aim to design and collect sentences that are representative in ASL.
%Furthermore, the words in these sentences should be also representatives of the ASL vocabulary.
%
%We design our ASL sentence dataset that follows three key design considerations:
% \squishlist{
% \item{Since it is impossible to collect all possible sentences in ASL, we aim to design and collect sentences that are representative to most, if not all, sentences in ASL. Furthermore, the words that construct these sentences must be also representatives of the whole ASL vocabulary.
% }
 %\item{Training our deep network large dataset which ought to contain enough variation in terms of gesture execution. We aim to collect a dataset that its size is larger or comparable to those of other state-of-the-art skeleton deep networks. 
 %}
% \item{In order to evaluate the generality of {\modeltwo} in recognizing sentences of different structures, we aim to design and collect a challenging testing dataset that the lengths of these sentences consist of different numbers of words from those of the training dataset. 
% }
 %\item{Datasets with imbalanced class distributions are quite common but might present problems to classification algorithm. Thus, we also aim to design and collect a dataset with relatively balanced occurrence of each word, yet not perfectly balanced so as to mimic a real world large scale training process. 
 %}
% }\squishend
%
We have followed the dataset design methodology used in Google's LipNet (i.e., sentence-level lipreading) \cite{assael2016lipnet} to design our ASL Sentences Dataset.
%
Specifically, we design the ASL sentences by following a simple sentence template: $subject^{(4)} + predicate^{(4)} +  attributive^{(4)} + object^{(4)}$, where the superscript denotes the number of word choices for each of the four word categories, which are designed to be $\lbrace I, you, mother, who \rbrace$, $\lbrace dontwant, like, want, need \rbrace$, $\lbrace big, small, cold, more \rbrace$ and $\lbrace time, \\ food, drink, clothes \rbrace$, respectively.
%
%The four categories are $\lbrace I, you, mother, who \rbrace$, $\lbrace dontwant, like$, $want$, $need \rbrace$, $\lbrace big, small, cold, more \rbrace$ and $\lbrace time, food, drink, clothes \rbrace$, respectively, generating a total $256$ sentences. 
%We selected these 16 words from top 200 most common words in ASL as they are representative of larger sets. 
%
Based on this sentence template, a total of $256$ possible sentences can be generated. 
%
%Unlike meaningless sentences used in Google's LipNet \cite{assael2016lipnet}, 
Out of these 256 sentences, we hand picked $100$ meaningful sentences that people would use in daily communication.
%
Example meaningful sentences are "I need more food" and "Who want cold drink".
%
% We then randomly selected {\numsen} sentences out of the hand picked 100 meaningful sentences to be our ASL Sentences Dataset. 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
\vspace{1mm}
\noindent
\textbf{In-the-Field Dataset}: 
%\textbf{Daily Communication Dataset}: 
%
In daily life, deaf people may need to use ASL to communicate with others under various real-world settings.
%
We consider three common real-world factors that can potentially affect the ASL translation performance: 1) lighting conditions, 2) body postures; and 3) interference sources. 
%
For lighting conditions, we collected data from both indoor poor lighting scenario and outdoor bright sunlight scenario. 
%\biyi {T7} 
%In particular, the camera sensors of iPhone 7 and Nikon DSLR both failed in the poor lighting conditions as we tested them. 
%
For body postures, we collected data when signs are performed while the signer stands or walks.
%
For interference sources, we considered two interference sources: people and device.
%
In terms of people interference, data was collected while another person stands in front of {\leap} with both of her hands appearing in the viewing angle of the {\leap} sensor. 
%spaced with social distance (i.e., 1.2 meters to 2.1 meters~\cite{karakayali2009social}) 
This setup simulates the communication scenario between a deaf person and a normal hearing person. 
%
In terms of device interference, data was collected while another person is wearing {\leap} standing near the user. 
%The interferer is instructed to orient her body to the user at various angles. 
%
This setup simulates the communication scenario where there are more than one person using {\sysname}.


%We collect a dataset where ASL words are collected under three communication conditions that will potentially affect the performance of {\sysname}. 
%The rationales and data collection process are:

%\squishlist{
 %\item{\textbf{Lighting Condition:} In order for its camera to see capture the images of hand clearly, {\leap} illuminates the target area by emitting infrared lights. As such, {\leap} is able to capture ASL even under the dark light condition. On the other hand, the fact that sunlight contain significant amount of infrared light might deteriorate the performance of {\sysname}. 
 %
 %Specifically, in the first scenario, we collect data inside a completely dark and window-less room while the monitor of the {\leap} host machine is dimmed to lowest light and placed far away from the device. In the second scenario, data is collected in an outdoor open space in the afternoon where there is sufficient daylight. Meanwhile, {\leap} camera is pointing an arbitrary background (e.g., mixture of building, tree or sky). 
 %}
 %\item{\textbf{Body Posture:} Similar to natural language, ASL can also be communicated under different postures (e.g., sitting, standing and walking). Therefore, the performance is potentially affected because of the change of start and stop hand positions (standing); or because of the constant change of background (walking). 
 %
 %Specifically, in the first scenario, data is collected while the participants are standing still. In the second scenario, data is collected while the participants are walking at a normal speed at indoor hallway.
 %}
 %\item{\textbf{Interference Source:} The ambient environment when using {\sysname} might introduce interference. Other people's hands in front of you might mistake {\leap}; Another {\leap} device might affect the hand recognition due to ambient infrared light confusion.  
%
%Specifically, in the first scenario, data is collected while another person standing in front of {\leap} spaced with social distance (i.e., 1.2 meters to 2.1 meters~\cite{karakayali2009social}) with both of her hands appearing in the viewing angle of the camera. This scenario simulates the deaf to normal person communication condition. In the second scenario, data is collected while another person (interferer) is wearing {\leap} standing near the participant with a social distance. This interferer is instructed to orient her body to the participant at various angles. This scenario simulates the communication conditions where there are more than one users are using {\sysname}.
 %}
 %}\squishend
 
%\begin{figure}[t]
%\centering
%\hspace{-1mm}
%\includegraphics[scale=0.285]{Images/eval/setup/mount.pdf}
%\vspace{-2mm}
%\caption{(a) 3D-printed rotational {\leap} mount; (b) Illustration of {\leap} setup when clipped on the upper chest of a user.}
%\vspace{-4mm}
%\label{dia.mount}
%\end{figure}  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
%\subsubsection{Participants and Data Collection Procedure}
\vspace{1mm}
\subsubsection{Participants}
~\newline
%%
%\noindent
%\textbf{\\Participants}: 
%
%Our study is approved under IRB i053743.
Our study is approved by IRB.
%
Due to the IRB constraint, we could only recruit people with normal hearing ability to participate in the study.
%As such, we first conducted a filtering round to select participants who are capable of performing the target ASL.
%After the approval of on-site IRB (No. i053743), we recruit 21 people via flyer advertisement. 
%21 participants were initially recruited.
%
We recruited 11 participants and hosted an 3-hour tutorial session to teach them how to perform the target ASL signs using online ASL tutorial videos.
%recruits were instructed to learn to perform ASL for at least 5 hours, following provided ASL tutorial videos. 
%By doing this, we make sure that these recruits have adequate knowledge of performing target ASL. 
%Next, participants were instructed to perform the target ASL words in front of a RGB camera while wearing {\leap}. We then sent the recorded RGB videos (third-person view) along with {\leap} videos (first-person view) to an ASL expert. 
%After evaluating the performance based on these two sets of videos, 11 out of 21 participants were selected by the ASL expert due to their competence of performing target ASL.
%
The 11 participants (four female) are between 20 to 33 ($\mu$ = 24.2) years old, weighted between 49 kg to 86 kg ($\mu$ = 74 kg) and are between 155 cm to 185 cm tall ($\mu$ = 173 cm). 


%%
%\vspace{1mm}
%\noindent
%\textbf{Data Collection Procedure}:
%
%Throughout the experiments, participants were requested to wear one {\leap} on their upper chest.
%To facilitate this, we have 3D-printed a plastic mount that can be clipped on the clothes of the participants. 
%As shown in Figure~\ref{dia.mount}(a), the mount has three functional parts: (1) an elastic mount that firmly holds {\leap}; (2) a mount clip; 
%to clip with that could hold onto the clothes of user tightly; 
%and 3) a rotational hinge that allows users to adjust the viewing angle of {\leap} to best capture ASL.
%and 3) a rotational hinge that allows users to enables the rotation of {\leap} so that users can adjust it to their customized viewing angle in order for camera to capture ASL. 
%Figure~\ref{dia.mount}(b) shows the setup where {\leap} is mounted onto a user's upper chest. 
%As shown, {\leap} fully covers the space in front of the user where ASL is performed. 

%%
%Figure~\ref{dia.datacollect} illustrates our data collection setup.
%During data collection, by default, participants were instructed to sit still and perform the ASL words and sentences. 
%During data collection, by default, participants were instructed to sit still in a window-less room (no ambient infrared light). 
%
%Meanwhile, {\leap} is connected to its USB host Microsoft Surface Pro 4. 
%
%To facilitate data collection, we have designed a user interface to help record and label data.
%We have also designed a data visualization tool to visualize skeleton data. 
%As will be discussed in section 8, we will make these tools publicly available as part of our ASL crowdsourcing initiative. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
%%
\vspace{1mm}
\subsubsection{Summary of Datasets}
~\newline
%
Table~\ref{tab.sum} summarizes the amount of data collected in the three datasets.
%
Specifically, for ASL Words Dataset, we collected 56 ASL words with 10 ($\pm$3) samples of each word from each of the 11 participants. 
%
In total, $3,068$ and $3,372$ samples of one-hand and two-hand ASL words were collected, respectively.
%
For ASL Sentences Dataset, we randomly collected 80 ($\pm$3) out of the $100$ meaningful sentences from each of the 11 participants.
%
In total, $866$ sentences were collected.
%
For In-the-Field Dataset, for each of the six scenarios, we randomly selected 25 out of the 56 ASL words and collected 3 ($\pm$1) samples of each word from three out of the 11 participants.
%
To the best of our knowledge, our datasets are the largest and the most comprehensive datasets in the sign language translation literature~\cite{kosmidou2009sign,dominio2014combining,uebersax2011real,zafrulla2010novel,melgarejo2014leveraging,brashear2003using}. 

%Training deep neural networks requires a large dataset. %which contains enough variation in terms of gesture execution. 
%
%and our datasets are comparable or larger than the datasets used for training deep neural networks that achieve state-of-the-art performance in similar recognition tasks~\cite{du2015hierarchical,rahmani2017learning,liu2016spatio,huang2016deep,ke2017new,song2017end}.
% In detail, we collected {\numsen} sentences from {\numsensub} participants with one to three repetition(s) of each sentence. 
%In detail, we collected {\numsen} randomly selected sentences (with replacement) from the hand picked 100 meaningful sentences to be our ASL Sentences Dataset.
%
% As shown in Figure ??, the occurrence of each word is balanced, ensuring a non-biased training of {\modeltwo}. 
%For each conditions, we collect data under two scenarios.

 



%\begin{figure}[t]
%\centering
%\hspace{-1mm}
%\includegraphics[scale=0.245]{Images/eval/datacollect.pdf}
%\vspace{-2mm}
%\caption{Experimental setup for data collection.}
%\vspace{-4mm}
%\label{dia.datacollect}
%\end{figure} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{-2mm}
\begin{table}[h]
\centering
\scalebox{0.83}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Category}    & \multicolumn{2}{c|}{\textbf{ASL Words}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{ASL}\\\textbf{Sentences} \end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textbf{In-the-} \\\textbf{Field}\end{tabular}} & \multirow{2}{*}{\textbf{Total}} \\ \cline{1-3}
Subcategory &\textbf{One-hand}           &\textbf{Two-hand}          &                                                                                    &                                                                                                       &                        \\ \hline
Duration (s)  &       7541.7           &    8616.3       &             5094.3
 &           2498.4                                                                                            &                       23750.7 \\ \hline
Frames      &     821846        &      949310     &                                                                                   507001 &                 259431         &       2537588      \\ \hline
Samples     &     
3068      &   3372   &          866                &                                                                                                      1178 &        8484         \\ \hline
\end{tabular}
}
\vspace{0mm}
\caption{Summary of datasets}
%The breakdown of the amounts of data collected for ASL Words, ASL Sentences, and In-the-Field Datasets.
\vspace{-8.5mm}
\label{tab.sum}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsubsection{Evaluation Metrics and Protocol}
\vspace{1mm}
\noindent
\textbf{\\Evaluation Metrics:} 
%
We use different metrics to evaluate the translation performance of {\sysname} at the word and sentence levels.
%
Specifically, at the word level, we use word translation accuracy, confusion matrix, and Top-$K$ accuracy as evaluation metrics. 
%At word level, we use average accuracy across all word classes as the metric. 
%Average accuracy is defined as:
%\begin{equation} 
%Accuracy = \frac{\Sigma TP_{i}}{\Sigma NS_{i}},~~~i = 1, ..., 25
%\end{equation}
%where $TP_{i}$ is true prediction of class $i$, and $NS_{i}$ is number of samples of class $i$. This metric essentially reflects the overall successful prediction rate of 25 ASL word
%The higher $Accuracy$ is, the better performance {\sysname} achieves.
%
%
At the sentence level, we use word error rate ($WER$) as the evaluation metric, which is defined as the minimum number of word insertions, substitutions, and deletions required to transform the prediction into the ground truth, divided by the number of words in the ground truth. 
%
$WER$ is also the standard metric for evaluating sentence-level translation performance of speech recognition systems.
%$WER$ is also the standard metric for evaluating sentence level translation performance of automatic speech recognition (ASR) systems.
%
%As the ASL sentence of {\sysname} is one kind of automatic speech recognition (ASR) systems, we evaluate the recognition performance of a single sentence by the word error rate ($WER$), standard metric for the performance of ASR. 
%
%Specifically, $WER$ is defined as:
%\begin{equation} 
%WER = \frac{S + D + I}{N}
%\end{equation}
%where $S$ is the number of substitutions, $D$ is the number of deletions, $I$ is the number of insertions, and $N$ is the number of words in ground truth. 
%In other words, $WER$ is defined as the minimum edit over the length of the ground truth. 
%As an example, if $WER$ is 25\% of a four-word sentence (i.e., $N$ = 4), it means that one edit (i.e., substitution, deletion or insertion) must be taken to correct the prediction. 
%As such, the lower $WER$ is, the higher the sentence-level recognition performance is. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
\vspace{1mm}
\noindent
\textbf{Evaluation Protocol:} 
%
At both word and sentence levels, we use leave-one-subject-out cross-validation as the protocol to examine the generalization capability of {\sysname} across different subjects. 
%At sentence level, we also use leave-one-subject-out cross-validation as the evaluation protocol. 
%
In addition, to evaluate the performance of {\sysname} in translating unseen sentences, we randomly divide ASL sentences into ten folds, making sure that each fold contains unique sentences to the rest nine folds. 
%
We then use ten-fold cross-validation as the protocol. 
%
%To evaluate the performance over all testing sentences, we use the average value of all $WER$ obtained from each single sentence.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
\centering
\hspace{-6mm}
\includegraphics[scale=0.53]{Images/eval/confusion27.pdf}
\vspace{-2mm}
\caption{Confusion matrix of 27 one-hand ASL words.}
\vspace{-1mm}
\label{dia.confusion27}
\end{figure} 

\begin{figure}[h]
\centering
\hspace{-5mm}
\includegraphics[scale=0.52]{Images/eval/confusion29.pdf}
\vspace{-2mm}
\caption{Confusion matrix of 29 two-hand ASL words.}
\vspace{-3mm}
\label{dia.confusion29}
\end{figure} 

%%  
%1
\begin{figure*}[t]
\captionsetup{width=0.31\textwidth}
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \vspace{-1mm}
        \includegraphics[width=0.99\linewidth, keepaspectratio]{Images/eval/word_sub.pdf}
         
        \caption{Word-level ASL translation accuracy across 11 participants.}
        \vspace{-2mm}
        \label{dia.word_sub}
    \end{minipage}%
    \hspace{3mm}
    \begin{minipage}{0.31\textwidth}
    \vspace{0mm}
        \centering
        \includegraphics[width=0.99\linewidth, keepaspectratio]{Images/eval/sen_rank_sub.pdf}
        \caption{Top-10 $WER$ in translating ASL sentences of unseen participants.}
       % \vspace{3.6mm}
        \label{dia.sen_rank_sub}
    \end{minipage}
    \hspace{3mm}
    \begin{minipage}{0.31\textwidth}
        \centering
        \vspace{0mm}
        \includegraphics[width=0.99\linewidth, keepaspectratio]{Images/eval/sen_rank_unseen.pdf}
      
        \caption{Top-10 $WER$ in translating unseen sentences.}
        \label{dia.sen_rank_unseen}
    \end{minipage}
    \vspace{-0mm}
\end{figure*}

%% Part 1
\subsection{Word-Level Translation Performance}
%As the first experiment for ASL translation, we evaluate the performance of {\sysname} in recognizing 25 ASL words. 
%
Figure~\ref{dia.word_sub} shows the average word-level ASL translation accuracy across 11 participants. 
%
Overall, {\sysname} achieves an average accuracy of $94.5\%$ on translating 56 ASL words across 11 participants. 
%
This is a very impressive result considering it is achieved based on leave-one-subject-out cross validation protocol. 
%
Further, we observe that the margin between the highest (participant\#1, 98.4\%) and the lowest (participant\#11, 90.6\%) accuracies is small. 
%
This indicates that our HB-RNN model is capable of capturing the key characteristics of ASL words. 
%
Furthermore, the standard deviation of these accuracies is as low as 2.4\%, which also demonstrates the generalization capability of our model across different users. 

%%
To provide a more detailed view of the result, Figure~\ref{dia.confusion27} and~\ref{dia.confusion29} show the confusion matrices of translating 27 one-hand ASL words and 29 two-hand ASL words, respectively. 
%
As shown in Figure~\ref{dia.confusion27}, among all the 27 one-hand ASL words, only \textit{please} (word\#20) achieves 100\% in both precision and recall. 
%
This is because \textit{please} has very distinctive hand shape and hand movement characteristics. 
%
In contrast, \textit{hot} (word\#9) achieves the lowest precision of 81.1\% and \textit{bad} (word\#21) achieves the lowest recall of 86.3\%.
%, indicating that it is more likely to misclassify other words into \textit{hot}. 
%Meanwhile, \textit{bad} (word\#21) achieves the lowest recall of 86.3\% where the majority of the samples are misclassified into either \textit{hot} or \textit{blue} (word\#9 and word\#10, respectively). 
%
Similarly, as shown in Figure~\ref{dia.confusion29}, among all the 29 two-hand ASL words, \textit{big} (word\#7) achieves 100\% in precision and \textit{bicycle} (word\#19) achieves 100\% in recall, whereas \textit{with} (word\#15) has the lowest precision of 90.7\% and \textit{but} (word\#29) has the lowest recall of 84.3\%.
%
%We observe that ASL word \textit{you}, \textit{like}, \textit{food}, \textit{help}, \textit{big} and \textit{box} (index 1, 5, 6, 18, 20 and 25, respectively) achieve 100\% in either precision or recall. Among them, only \textit{help} achieves 100\% in both precision and recall. This is because these ASL words have relatively distinctive patterns in terms of hand shape and movement. At the same time, we observe that there is a major confusion between word \textit{need} and \textit{where} (index 4 and 13, respectively) where there are 14 out of 111 \textit{where} samples are misclassified into \textit{need}. Another major confusion happens on \textit{cold} (index 19) where 10 and 9 out of 110 samples are misclassified into either \textit{more} or \textit{big} (index 17 and 20, respectively). This is because these two sets ASL words are intrinsically similar in terms of hand shape and movement. %, see Figure XX for clarification. 



%Above all, {\sysname} shows promising results in ASL word recognition and thus indicates the great promise of expanding ASL vocabulary into a large scale.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{The Necessity of Model Components}

%%
To validate the design choice of our proposed HB-RNN model, we compare the translation performance between HB-RNN and four comparative models introduced in section 5.2.3.
%
To make a fair comparison, we set the number of hidden units of each model such that the total number of parameters of each model is roughly the same. 
%
We use the ASL Words Dataset to evaluate these models. 
%and report the accuracy of top-3 ranks ASL word prediction. 
%We use leave-one-subject-out cross validation as evaluation protocol. 
%
Table~\ref{tab.compare} lists the evaluation results in terms of average Top-$K$ ($K = 1,2,3$) accuracies and standard deviations across 11 participants.
% of four comparative models along with our model. 
%
As listed, our proposed HB-RNN model outperforms all four comparative models across all three Top-$K$ metrics. 
%
Specifically, our HB-RNN model achieves an 5.1\%, 5.0\%, 3.4\% and 0.8\% increase in average Top-$1$ accuracy over the four comparative models, respectively. 
%
This result demonstrates the superiority of our HB-RNN model over the four comparative models.
%It is important to note that although an 0.8\% increase over the H-RNN model seems small, given that H-RNN has already achieved a high average Top-$1$ accuracy of 93.7\%, achieving an 0.8\% increase is much harder than that when the accuracy is low.	
%it actually shows a substantial advantage of bidirectional connection. 
%
It also indicates that the hand shape information, hand movement information, the hierarchical structure, as well as the bidirectional connection capture important and complimentary information about the the ASL signs.
%
By combining these important and complimentary information, the best word-level translation performance is achieved.
%Moreover, our model achieve lowest overall standard deviation of accuracy.%, meaning that it is more robust to performed ASL variation among 11 participants. 
%Equally important, we observe that the two models with either only trajectory or hand shape achieves an average accuracy above 90\%, indicating that both trajectory and hand shape capture the core information of a performed ASL. %Lastly, the top-3 rank performance of our model is very close to 100\%, which indicates {\sysname} has great potential.


%In other words, our model is capable of learning and capturing the information of ASL.

\begin{table}[h]
\centering
\scalebox{0.74}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Model}     &\textbf{ Top-1 (\%) }   &\textbf{ Top-2 (\%)  }  &\textbf{ Top-3 (\%)  }  & \textbf{Note}      \\ \hline
HB-RNN-M & 89.4 $\pm$ 3.1 & 95.4 $\pm$  1.8 & 97.2 $\pm$ 1.2 & No hand shape    \\ \hline
HB-RNN-S & 89.5 $\pm$ 2.4 & 94.9 $\pm$ 1.7 & 97.0 $\pm$ 1.3 & No hand movement    \\ \hline
SB-RNN   & 91.1 $\pm$ 3.4 & 96.5 $\pm$ 1.7 & 98.2 $\pm$ 1.2 & No hierarchical structure    \\ \hline
H-RNN    & 93.7 $\pm$ 1.7 & 97.1 $\pm$ 0.9 & 98.1 $\pm$ 0.6 & No bidirectional connection   \\ \hline
\textbf{HB-RNN}  &\textbf{ 94.5 $\pm$ 2.4} & \textbf{97.8$\pm$ 1.3}& \textbf{98.7 $\pm$ 0.9}& \textbf{Our model }\\ \hline
\end{tabular}
}
\vspace{2mm}
\caption{Comparison of word-level ASL translation performance between HB-RNN and four comparative models.}
\vspace{-7.5mm}
\label{tab.compare}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Sentence-Level Translation Performance}
\vspace{1mm}
\subsubsection{Performance on Unseen Participants}
%In this experiment, we evaluate the performance of our ASL sentence recognition model. 
~\newline
We first evaluate the performance of DeepASL on translating ASL sentences using leave-one-subject-out cross-validation protocol. 
%
Figure~\ref{dia.sen_rank_sub} shows the results in Top-10 $WER$. 
%The error bar means that the $WER$ standard deviation across 11 participants. 
%
Specifically, the Top-1 $WER$ is 16.1 $\pm$ 3.7\%. 
%
It indicates that for a 4-word sentence, there is only an average 0.64 words that needs either substitution, deletion or insertion. 
%
This is a very promising results considering: 1) there are 16 candidate classes (16 ASL words that construct these sentences) in each frame of the sequence; 2) we do not restrict the length or the word order of the sentence during inference and thus there is an enormous amount of possible label sequences; and 3) no language model is leveraged to help improve the performance.
%Moreover, we observe that the Top-4 $WER$ is 5.1 $\pm$ 3.1\%. 
%This indicates that our model can achieve very high sentence-level translation performance without any restriction and language model. 
%We note that adding language model may lead to a significant recognition performance boost. But this paper focuses on evaluating the feasibility of ASL sentence recognition using our hierarchical bidirectional RNN, the additional implementation of language model is out of scope, and we will leave it to future work.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{1mm}
\subsubsection{Performance on Unseen Sentences}
%
~\newline
We further conduct an experiment to evaluate the performance of DeepASL on translating unseen sentences (i.e., sentences not included in the training set). 
%We aim to find the performance of {\sysname} in recognizing ASL sentences with the addition of personalized data. 
%
The results are illustrated in Figure~\ref{dia.sen_rank_unseen}.
% shows the top-10 ranks $WER$ of {\sysname} in recognizing unseen sentences. 
%
%Specifically, the Top-1, Top-4 and Top-10 $WER$ is 8.2 $\pm$ 5.4\%, 1.8 $\pm$ 2.2\% and 0.4 $\pm$ 0.8\%, respectively. 
Specifically, the Top-1 $WER$ is 8.2 $\pm$ 5.4\%. 
%
This indicates that there is only an average 0.33 out of 4 words that needs substitution, deletion and insertion. 
%
This is a very promising result considering that the translated sentences are not included in the training set.
%
As a result, it eliminates the burden of collecting all possible ASL sentences.
% trained model has never encountered the target sentence. 
%We also observe that there is an significant performance increase comparing to the result of unseen participants. 
%This is because the training set consists of the sentences from all participants and thus contains the ASL characteristics performed by all participants. 
%As such, the trained model would better model the performance of each participant and generate better results. 
%This indicates that instead of modeling the entire sentence, CTC models the probabilistic dependencies between words and thus able to predict sentence that is not in the training set.
%Therefore, we demonstrate that, with limited amount of unique sentences available, our CTC-based framework is capable of translating unseen sentences as long as the framework has encountered all words in one particular unseen sentence.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Robustness of ASL Translation in the Field}
%
Table~\ref{tab.scenario} lists the word-level ASL translation performance achieved on the In-the-Field Dataset.
%In this experiment, we evaluate the robustness of {\sysname} in ASL word recognition. The objective is to discover how robust {\sysname} can be under daily communication scenarios. Equally important, this experiment also involve scenarios where other ASL sensing modalities might fail. In detail, we use the data collected from three participants as testing data and the data of ASL words as training data. By doing this, we could find the impact of each scenario on the performance of {\sysname} and how generalized our ASL word dataset can be. We present three parts of results.

\vspace{1.5mm}
\noindent
\textbf{Impact of Lighting Conditions:} 
%
Under poor lighting condition, {\sysname} achieves 96.8 $\pm$ 3.1\% accuracy. 
%
It indicates that the poor lighting condition has very limited impact on the performance of {\sysname}. 
%
Under outdoor sunlight condition, {\sysname} achieves 91.8 $\pm$ 4.1\% accuracy. 
%
This result indicates that the significant portion of infrared light in the sunlight also has very limited impact on the performance of {\sysname}.
%This is due to the fact that {\leap} is designed to automatically remove bright background so as to work in outdoor environment. 

\vspace{1.5mm}
\noindent
\textbf{Impact of Body Postures:} {\sysname} achieves 92.2 $\pm$ 3.0\% and 94.9 $\pm$ 4.5\% on walking and standing postures, respectively. The accuracy only drops slightly comparing to previous ASL word recognition result, indicating that {\sysname} could also capture information with either standing or sitting body posture. Moreover, this result also demonstrates the advantage of {\leap} over inertial sensors which are very susceptible to human body motion artifacts.

\vspace{1.5mm}
\noindent
\textbf{Impact of Interference Sources:}  {\sysname} achieves 94.7 $\pm$ 3.0\% and  94.1 $\pm$ 1.3\% on people in-the-scene interference and multi-device interference, respectively. In the first scenario, the accuracy is comparable to previous ASL word recognition result, meaning that {\sysname} is robust to this two interference scenarios. 
%
We observe that spaced with social distance, {\leap} is rarely confounded by the hands of an interferer. This is because the cameras of {\leap} both have fish-eye angle view, making the far objects too small to be detected. 
%
As a matter of fact, effective range of {\leap} is designed to be no more than approximately 80 cm~\cite{leapapi}, much less than the social distance. 
%
On the other hand, our system is not affected by multiple {\leap} present in the ambient environment, indicating that {\sysname} is robust when multiple devices are being used at the same time. 
%
This is because {\leap} only uses infrared to illuminate the space where ASL is performed and hence the illumination does not have impact on the infrared images captured by the sensor.
%On the contrary, the depth sensor, either depending on Time-of-Flight (ToF) or structured light will suffer in this scenario.

%Above all, {\sysname} achieves accuracies in recognizing ASL words under six ASL daily communication scenarios. It means that {\sysname} is indeed robust to various real life conditions. Moreover, since these six scenarios do not essentially change the modeling process, we argue that these results fully reveal the potential of {\sysname}, and are also representative to ASL sentence recognition. Thus, we will leave this to future work. 

\begin{table}[h]
\centering
\vspace{1mm}
\scalebox{0.70}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Category}    		& \multicolumn{2}{c|}{\textbf{Lighting}} & \multicolumn{2}{c|}{\textbf{Body}} & \multicolumn{2}{c|}{\textbf{Interference}} \\ 
\textbf{}    		& \multicolumn{2}{c|}{\textbf{Condition}} & \multicolumn{2}{c|}{\textbf{Posture}} & \multicolumn{2}{c|}{\textbf{Source}} \\ \hline
Subcategory 		& Poor             & Bright            & Walk            & Stand           & People          & Device          \\ \hline
Accuracy (\%)    	&  96.8 $\pm$ 3.1& 91.8 $\pm$ 4.3& 92.2 $\pm$ 3.0& 94.9 $\pm$ 4.5 & 94.7 $\pm$ 3.4 & 94.1 $\pm$ 1.3 \\ \hline
\end{tabular}
}
\vspace{2mm}
\caption{In-the-field ASL translation performance.}
\vspace{-5.5mm}
\label{tab.scenario}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Part 2
%\vspace{1mm} 






\subsection{System Performance}

%%
To examine the system performance, we have  implemented {\sysname} on three platforms with five computing units: 1) desktop CPU and GPU, 2) mobile CPU and GPU, and 3) tablet CPU. 
%(Figure~\ref{dia.platform}). 
%
Our goal is to profile the system performance of {\sysname} across platforms with different computing powers. 
%
Specifically, we use a desktop installed with an Intel i7-4790 CPU and a Nvidia GTX 1080 GPU to simulate a cloud server; 
%
we use a mobile development board that contains an ARM Cortex-A57 CPU and a Nvidia Tegra X1 GPU to simulate augmented reality devices with built-in mobile CPU/GPU\footnote{Since Mircrosoft Hololens currently does not support hosting USB clients, we could not implement {\sysname} in  Mircrosoft Hololens to test its system performance.}; 
%
and we use Microsoft Surface Pro 4 tablet and run {\sysname} on its Intel i5-6300 CPU. 
%
The specs of the computing units are listed in Table\ref{tab.test_beds}. 
%The pictures of these platforms are shown in Figure~\ref{dia.platform}.


%%
%We will not test the system performance on this platform because Hololens can not host USB client. 

%\begin{figure}[tb]
%\centering
%\includegraphics[scale=0.28]{Images/impl/platform.pdf}
%\caption{(a) Desktop (b) Mobile and (c) Tablet Platforms.}
%\vspace{-2mm}
%\label{dia.platform}
%\end{figure} 


%%In this section, we evaluate the system performance of {\sysname} on the three platforms illustrated in Figure~\ref{dia.platform}.
%To provide a comprehensive evaluation, we evaluate the system performance of three models: 1) one-hand ASL word translation model; 2) two-hand ASL word translation model; and 3) ASL sentence translation model.  
%
%We define the process \textit{from one ASL word/sentence is finished performing by one user to the return by our system} as a \textit{inference}. 
%In the following, we report their runtime performance, runtime memory performance, and power consumption performance.

To provide a comprehensive evaluation, we evaluate the system performance of three models: 1) one-hand ASL word translation model; 2) two-hand ASL word translation model; and 3) ASL sentence translation model.
%
In the following, we report their system performance in terms of runtime performance, runtime memory performance, and energy consumption. 
%In the following, we report their system performance respectively.


\vspace{-2.5mm}
\begin{table}[h]
	\centering
	\vspace{2mm}
	\scalebox{0.82}{
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{\textbf{Platform}} & \multicolumn{2}{c|}{\textbf{CPU}} & \multirow{2}{*}{\textbf{RAM}} & \multicolumn{3}{c|}{\textbf{GPU}} \\ \cline{2-3} \cline{5-7} 
		& \textbf{Cores} & \textbf{Speed} &  & \textbf{Cores} & \textbf{GFLOPS} & \textbf{Speed} \\ \hline
		Desktop & 8 & 3.6GHz & 16GB & 2560 & 8228 & 1.67GHz \\ \hline
		Mobile  & 4 & 1.9GHz & 4GB & 256 & 512 & 1GHz \\ \hline
		Tablet & 2 & 2.4GHz & 4GB & - & - & \multicolumn{1}{c|}{-} \\ \hline
	\end{tabular}
	}	
	\vspace{2mm}
	\caption{The specs of the three hardware platforms.}
	\label{tab.test_beds}
	\vspace{-7.5mm}
\end{table}  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
\subsubsection{Runtime Performance}
%%
~\newline
An \textit{inference} contains two parts: data fetching/preprocessing and forward feeding of deep network. Because the time consumed by data fetching/preprocessing is negligible comparing to forward feeding, we report only total \textit{inference} time. 
%
We run 200 ASL word/sentence recognition and report the average runtime performance. 
%
The results of runtime performance of three models on five computing units of three platforms are shown in Figure~\ref{dia.runtime}. To give a straightforward view, we order the time cost in an ascending order. 
%
At a high level, \textit{inference} takes much longer when running on the CPUs than on the GPUs across three models. 
%
In detail, PC-CPU is 8$\times$ to 9$\times$ faster than PC-GPU; TX1-CPU is 14$\times$ to 28$\times$ faster than TX1-GPU. There are two reasons: (1) during inference, only one sample is passing through the network, which substantially limits the component eligible for parallel computation; and (2) our models are built on RNN, meaning that its time-dependency nature intrinsically eliminate the possibility of parallelism. Therefore, we argue that during inference CPUs are better choice than GPUs. As such, {\sysname} does not need high-end GPU to do inference. 
%\biyi {T9} 
%
It is also worth pointing out that the runtime of ASL sentence recognition is longer than word recognition. This is because HB-RNN-CTC for sentence recognition has about twice as many parameters as HB-RNN for word recognition. 
%
Equally important, we observe that the time cost on all three CPUs are less than 282 ms (ASL sentence recognition on TX1-CPU) which means {\sysname} achieves \textit{real-time} recognition performance.
%

\begin{figure}[h]
\centering
\vspace{-1mm}
\includegraphics[scale=0.75]{Images/eval/runtime.pdf}
\vspace{-2mm}
\caption{Runtime performance of the three models.}
\vspace{-2mm}
\label{dia.runtime}
\end{figure} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
\subsubsection{Runtime Memory Usage}
%%
~\newline
Next we report the memory cost on various platforms in CPU and GPU mode. Again, we briefly report the average memory usage on three models. Because memory allocation highly depends on operating system and it is difficult to unravel the memory usage for each part, we only report the total memory usage of each model. For all three platforms, we report physical RAM usage and GPU memory usage.
We report these usages because they reflect the memory cost of each model and  might indicate the potential improvements. To clearly reflect the influence of three models on CPU, we report the RAM usage that is subtracted by the RAM usage before doing \textit{inference}. The total RAM usage without loading our model is $2891$ MB on desktop, $931$ MB on TX1 and $1248$ MB on Surface. 
%
%However, to the best of our knowledge, Tensorflow (Version 1.0.1) does not support explicit memory cost monitoring since by default, it reserves all GPU memory when running. Thus, to estimate the GPU memory cost of each model, we keep shrinking the allocated GPU memory to run our inference until Tensorflow reports out-of-memory. 
%
Figure~\ref{dia.memory} shows the memory cost on five computing units of three platforms. We observe that memory cost of ASL sentence \textit{inference} is larger than two hand ASL word \textit{inference}, which is larger than one hand ASL word. The reason is that in the ASL sentence model, there are more hidden units, thus demanding more allocated memory.

\begin{figure}[h]
\hspace{1.1mm}
\centering
\includegraphics[scale=0.75]{Images/eval/memory.pdf}
\vspace{-2mm}
\caption{Runtime memory usage of the three models.}
\vspace{-2mm}
\label{dia.memory}
\end{figure} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Energy Consumption}
%
~\newline
To evaluate the power consumption of {\sysname}, we use PWRcheck DC power analyzer \cite{pwrcheck} to measure the power consumption of both TX1 and Surface tablet. 
%Note that during testing, we turn off the battery-charging of Surface tablet in order to get accurate readings of power consumption. 
We run 200 ASL word/sentence recognition and report the average power consumption.
%
Table~\ref{tab.consumption} lists the average power consumption of TX1 and Surface respectively. 
%
We report the power consumption of TX1 to simulate augmented reality devices because the TX1 is designed for mobile device real-time artificial intelligence performance evaluation and thus reflects the portion of power consumed by \textit{inference} in augmented reality devices.
%
We observe that for TX1 the power consumption of performing inference on GPU is much larger than CPU. This is because: (1) due to the RNN structure of our model, limited amount of computation can be parallelled, making GPU is less efficient in inference than CPU; and (2) performing inference on GPU also involves processing on CPU (for data loading etc.) and thus costs almost twice as much power as CPU alone. 

% As shown, the power consumption of GPU is much larger than CPU as it not only takes more time to do \textit{inference}, but also consumes approximately twice as much power as well (why???). This 


\begin{table}[h]
\centering
\scalebox{0.83}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Platform}}                   & \multirow{2}{*}{\textbf{Task}}                 & \textbf{Power} & \textbf{Time} & \textbf{Energy} \\ 
                  &                 & \textbf{(W)} & \textbf{(ms)} & \textbf{(mJ)} \\ \hline
\multirow{7}{*}{\textbf{TX1}}     & Idle                  & 3.54     & -         & -           \\ \cline{2-5} 
                         & One-hand ASL word (CPU)   & 5.92     & 42.9       & 254.0      \\ \cline{2-5} 
                         & Two-hand ASL word (CPU) & 6.13     & 66.1     & 417.5      \\ \cline{2-5} 
                         & ASL sentence (CPU)        & 6.02     & 281.7     & 1695.8      \\ \cline{2-5} 
                         & One-hand ASL word (GPU)   & 12.31    & 746.2       &9185.7     \\ \cline{2-5} 
                         & Two-hand ASL word (GPU)  & 12.16    & 1943.4     &23631.7     \\ \cline{2-5} 
                         & ASL sentence (GPU)        & 11.75    & 4153.6   & 48804.8     \\ \hline
\multirow{6}{*}{\textbf{Surface}} & Sleep                 & 1.63     & -         & -           \\ \cline{2-5} 
                         & Screen-on             & 8.32     & -         & -           \\ \cline{2-5} 
                         & ASL Dictionary App-on     & 15.75    & -         & -           \\ \cline{2-5} 
                         & One-hand ASL word         & 23.67    & 26.1      & 591.7      \\ \cline{2-5} 
                         & Two-hand ASL word        & 24.21    & 52.7       &1117.8      \\ \cline{2-5} 
                         & ASL sentence              & 22.13    & 156.2     & 3456.7      \\ \hline
\end{tabular}
}
\vspace{2mm}
\caption{Energy consumption on TX1 and Surface.}
\vspace{-6.5mm}
\label{tab.consumption}
\end{table}

%%
Finally, in Table~\ref{tab.num_infer}, we report the estimated number of ASL word/sentence recognition that can be completed by TX1 and Surface, using fully-charged battery of Hololens (16.5 Wh) and Surface (38.2 Wh), respectively.
%
For TX1, the number of inferences of CPU is 36$\times$, 57$\times$ and 29$\times$ larger than those of its GPU for three model respetively. It means that in terms of performing \textit{inference}, CPU is more suitable. Meanwhile, despite the power consumption from other sources, a Hololens/Surface equal volume battery could support enough number of inferences within one day.


\begin{table}[h]
\centering
\scalebox{0.83}{
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Platform}                 & \textbf{Task}           & \textbf{CPU}    & \textbf{GPU}  \\ \hline
\multirow{3}{*}{\textbf{TX1}}     & One-hand ASL word & 233888 & 6467 \\ \cline{2-4} 
                         & Two-hand ASL word & 142291  & 2514 \\ \cline{2-4} 
                         & ASL sentence       & 35028  & 1217 \\ \hline
\multirow{3}{*}{\textbf{Surface}} & One-hand ASL word  & 232420  & -    \\ \cline{2-4} 
                         & Two-hand ASL word & 123031  & -    \\ \cline{2-4} 
                         & ASL sentence       & 39784  & -    \\ \hline
\end{tabular}
}
\vspace{2mm}
\caption{Estimated number of inferences on TX1 and Surface with a 16.5 Wh (Hololens) and 38.2 Wh (Surface) battery, respectively.}
\vspace{-7.5mm}
\label{tab.num_infer}
\end{table}





==> ASL_CR - Copy/intro.tex <==
%!TEX root = sensys2017.tex

\section{Introduction}
\label{sec.intro}

\begin{figure*}[tb]
\vspace{-2mm}
\centering
\includegraphics[scale=0.55]{Images/intro/sketch.pdf}
\vspace{-1.0mm}
\caption{Illustration of an envisioned scenario of real-time two-way communication enabled by {\sysname}: (a) {\sysname} translates the signs performed by the deaf person into spoken English and broadcasts the translated ASL sentence via a speaker; (b) {\sysname} captures the signs in a non-intrusive manner; (c) {\sysname} leverages the speech recognition technology to translate spoken English into texts, and projects the texts through a pair of augmented reality (AR) glasses.}
\vspace{-3.5mm}
\label{fig:vision}
\end{figure*} 

\noindent
%% P1: Talk about the deaf community and their inability to communicate with people who cannot understand ASL.
%
In the United States, there are over 28 million people considered deaf or hearing disabled~\cite{deafstats1}.
%
American Sign Language, or ASL in short, is the primary language used by deaf people to communicate with others~\cite{deafstats2}.
% 
Unfortunately, very few people with normal hearing understand sign language.
%
Although there are a few methods for aiding a deaf person to communicate with people who do not understand sign language, such as seeking help from a sign language interpreter, writing on paper, or typing on a mobile phone, each of these methods has its own key limitations in terms of cost, availability, or convenience.
%For example, for children who are born deaf and use sign language as their native language, writing English on a paper or typing English on a phone -- a task that is so simple for normal hearing people who are communicated using English from birth -- could be extremely challenging simply because English is not their native language.  
%In such case, having sign language interpreters would be very helpful. 
%However, hiring interpreters could be very expensive, and they are not always available when needed. 
%
As a result, there is an undeniable communication barrier between deaf people and hearing majority. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%% P2: Introduce ASL translation technology as the solution to this problem. Talk about existing work and their drawbacks.
%
At the heart of tearing down this communication barrier is the sign language translation technology.
%
Sign language is a language like other languages but based on signs rather than spoken words.
%
A sign language translation system uses sensors to capture signs and computational methods to map the captured signs to English.
%ASL is a language expressed by signs made by moving hands.
%The hand shape, movement and the relative location of two hands altogether encode the meaning of the sign language.
%
Over the past few decades, although many efforts have been made, sign language translation technology is still far from being practically useful.
% due to limitations in both sensing technology and computational methods.
%In terms of sensing technology, 
Specifically, existing sign language translation systems use motion sensors, Electromyography (EMG) sensors, RGB cameras, Kinect sensors, or their combinations~\cite{starner1998real, brashear2003using, wu2015real, li2012sign, chai2013visualcomm} to capture signs. 
%
Unfortunately, these systems are either intrusive where sensors have to be attached to fingers and palms of users, lack of resolutions to capture the key characteristics of signs, or significantly constrained by ambient lighting conditions or backgrounds in real-world settings.
%In terms of computational methods, the vocabulary of ASL contains thousands of individual signs. 
%Existing computational methods are not capable of handling such large number of signs and thus fail when the scale is increased considerably.
%
More importantly, existing sign language translation systems can only translate a single sign at a time, thus requiring users to pause between adjacent signs.
%
These limitations significantly slow down face-to-face conversations, making those sign language translation systems much less useful in daily-life communication scenarios.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%% P3: Talk about our vision on what the ultimate ASL translation technology would look like.
%
In this paper, we present \textit{{\sysname}}, a transformative deep learning-based sign language translation technology that enables non-intrusive ASL translation at both word and sentence levels.
%
%{\system} uses the {\leap} sensor ~\cite{leapmotion} -- a combination of two infrared cameras and three infrared LEDs -- to track the skeletons of the fingers, palms and forearms to capture the signs performed by a deaf person. 
%
{\sysname} can be embedded inside a wearable device, a mobile phone, a tablet, a laptop, a desktop computer, or a cloud server to enable ubiquitous sign language translation.
% 
As such, {\sysname} acts as an \textit{always-available virtual sign language interpreter}, which allows deaf people to use their primary language to communicate with the hearing majority in a natural and convenient manner.
%
As an example, Figure~\ref{fig:vision} illustrates an envisioned scenario where {\sysname} is in the form of a wearable device, enabling a deaf person and a hearing individual who does not understand ASL to use their own primary languages to communicate with each other face to face.
%real-time two-way communication between a deaf person and a hearing individual who does not understand ASL. 
%As illustrated in \textbf{Figure~\ref{fig:vision}}, we envision {\system} to be in the wearable form, which enables real-time two-way communications between a deaf person and a hearing individual who does not understand ASL. 
%
Specifically, from one side, {\sysname} translates signs performed by the deaf person into spoken English; from the other side, {\sysname} leverages the speech recognition technology to translate English spoken from the hearing individual into text, and projects the text through a pair of augmented reality (AR) glasses for the deaf person to read. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%% P4: Overview of our work and its key innovations. Describe how our work overcomes the drawbacks of existing technologies.
% 1. Talks about what it is at a very high level: 
% 2. Talks about its 2 key innovations: 
%In this work, we make the first step towards turning this vision into reality by presenting \textit{{\sysname}}, an innovative wearable system that enables unobtrusive ASL translation at both word and sentence levels in real time.
%
{\sysname} uses {\leap}~\cite{leapmotion} -- an infrared light-based sensing device that can extract the skeleton joints information of fingers, palms and forearms -- to non-intrusively capture the ASL signs performed by a deaf person. 
%
By leveraging the extracted skeleton joints information, {\sysname} achieves word and sentence-level ASL translation via three innovations. 
%
First, {\sysname} leverages domain knowledge of ASL to extract the key characteristics of ASL signs buried in the raw skeleton joints data.
%
Second, {\sysname} employs a novel hierarchical bidirectional deep recurrent neural network (HB-RNN) to effectively model the spatial structure and temporal dynamics of the extracted ASL characteristics for word-level ASL translation.
%Second, {\sysname} employs a novel hierarchical bidirectional deep recurrent neural network (HB-RNN) to effectively combine the isolated and unorganized low-level ASL characteristics into an integrated high-level representation for word-level ASL translation.
% that models the spatial structure and temporal dynamics of the spatio-temporal trajectory of ASL characteristics for word-level ASL translation.
%for ASL translation at the word level. 
%Second, {\sysname} employs a novel hierarchical bidirectional recurrent neural network (HB-RNN) for word-level ASL translation. 
%The HB-RNN effectively combines the isolated ASL characteristics of both hands into an integrated representation for ASL recognition at the word level. 
%
%\biyi {T8} 
%
Third, {\sysname} adopts a probabilistic framework based on Connectionist Temporal Classification (CTC)~\cite{graves2006connectionist} for sentence-level ASL translation.
%that captures probabilistic dependencies between words contained in one complete sentence. 
%
This eliminates the restriction of pre-segmenting the whole sentence into individual words, and thus enables translating the whole sentence end-to-end directly  without requiring users to pause between adjacent signs. 
%
%Our proposed sentence-level ASL translation approach addresses the key limitation of the existing sign language translation systems and, therefore, is able to translate the whole sentence without requiring users to pause between adjacent signs. This advancement marks a significant milestone towards realizing the envisioned natural communication between deaf and hearing.
%
%\biyi {T2} 
%More importantly,
Moreover, it enables {\sysname} to translate ASL sentences that are not included in the training dataset, and hence eliminates the burden of collecting all possible ASL sentences.   


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\vspace{1.5mm}
%% P5: Summary of Experimental Results.
\noindent
\textbf{Summary of Experimental Results:}
%%
We have conducted a rich set of experiments to evaluate the performance of {\sysname} in three aspects: 
%
1) ASL translation performance at both word level and sentence level; 
%
%2) robustness of ASL translation under various daily communication scenarios; 
2) robustness of ASL translation under various real-world settings; 
%
and 3) system performance in terms of runtime, memory usage and energy consumption. 
%
Specifically, to evaluate the ASL translation performance, we have collected $7,306$ samples from $11$ participants, covering $56$ commonly used ASL words and $100$ ASL sentences.
%
To evaluate the robustness, we have collected $1,178$ samples under different ambient lighting conditions, body postures when performing ASL, and scenarios with in-the-scene interference and multi-device interference. 
%
%To evaluate the system performance, we have implemented {\sysname} on five computing units of three hardware platforms with different computing powers: 1) desktop CPU and GPU, 2) mobile CPU and GPU, and 3) tablet CPU.
% 
To evaluate the system performance, we have implemented {\sysname} on three platforms with different computing power: 1) a desktop equipped with an Intel i7-4790 CPU and a Nvidia GTX 1080 GPU (desktop CPU and GPU), 2) a Nvidia Jetson TX1 mobile development board equipped with an ARM Cortex-A57 CPU and a Nvidia Tegra X1 GPU (mobile CPU and GPU), and 3) a Microsoft Surface Pro 4 tablet equipped with an Intel i5-6300 CPU (tablet CPU).
%
Our results show that:
%
\squishlist{
\item{
%
At the word level, {\sysname} achieves an average $94.5\%$ translation accuracy. 
%
At the sentence level, {\sysname} achieves an average $8.2\%$ word error rate on translating unseen ASL sentences and an average $16.1\%$ word error rate on translating ASL sentences performed by unseen users. 
} 
%
\item{
%
{\sysname} achieves more than $91.8\%$ word-level ASL translation accuracy in various ambient lighting conditions, body postures, and interference sources, demonstrating its great robustness in real-world daily communication scenarios.
}

\item{{\sysname} achieves $282$ ms in runtime performance in the worst-case scenario across three platforms for both word-level and sentence translation. 
%
It also demonstrates the capability of supporting enough number of inferences for daily usage on both mobile and tablet platforms.  

}
}\squishend


\vspace{1.5mm}
%% P6: Summary of technical contributions and its broader impact.
\noindent
\textbf{Summary of Contributions:}
%% Summary of technical contributions
%In this work, we introduce {\sysname}, a novel wearable system that is able to accurately translate ASL at both word and sentence levels in real time.
% the first system that is able to translate ASL at both word and sentence levels with real-world applicable recognition performance.
%
The development of sign language translation technology dates back to the beginning of 90s~\cite{von2008recent}.
%
However, due to the limitations in both sensing technology and computational methods, limited progress has been made over the decades.
%, and none of the sign language translation systems currently found in literature meets the requirements for robust real-world applications~\cite{von2008recent}. 
%there was virtually no technological breakthrough achieved over the decades, and none of the sign language translation systems currently found in literature meets the requirements for real-time word-level and sentence-level ASL translation applications~\cite{von2008recent}. 
%
The innovative solution provided by {\sysname} effectively addresses those limitations, and hence represents a significant contribution to the advancement of sign language translation technology.
%We deeply believe that, with that considerable advancement, we could turn the ultimately vision of tearing down the communication barrier between the deaf people and the hearing majority into reality.
%
Moreover, the development of {\sysname} enables a wide range of applications. 
% 
As another contribution of this work, we have designed and developed two prototype applications on top of {\sysname} to demonstrate its practical value. 
% For the first application, we will develop a wearable system called MyVirtualInterpreter, which aims to enable natural face-to-face communication between a deaf person and a person with normal hearing as illustrated in Figure 1. For the second application, we will develop a tablet application called MyASLTutor, which aims to help the hearing parents of deaf children to learn ASL.
%
%To demonstrate the usage scenarios of {\sysname}, we have implemented two prototype applications: 
%1) \textit{Personal Interpreter}: a Microsoft Hololens application that focuses on realizing real-time two-way communication between deaf and normal persons;
%and 2) \textit{ASL Dictionary}: a tablet application that focuses on helping a deaf person look up any unknown ASL word easily.
%
%% Talk about our initiative on crowdsourcing
%
%The dataset we collected during the development of {\sysname} is the largest among its kind. With the vision of making {\sysname} being able to recognize all the words in ASL vocabulary and many more sentences that deaf people use in their daily-life communications, we have taken an initiative on sign language data crowdsourcing. We have made our dataset and data collection toolkit publicly available (\url{http://goo.gl/krtGr3}). We hope our contribution can act as a seed for the development of a community of the same vision as we have, and to turn this vision into reality. We deeply believe that, with the crowdsourced efforts, we can collectively make a significant contribution to our society.



% We only target a subset of ASL. To realize the ultimate goal, we realize it requires collective efforts. Thus, we have made our dataset and data collection toolkit public available. We hope this work can act as a seed for the development of a community with the same vision as we have, to collectively contribute the data and make the ultimate goal into reality.

%% Broader impact
%While the focus of this paper is on American sign language translation, our approach can be tailored to recognizing other sign languages as well.
%
According to World Health Organization (WHO), there are an estimated 360 million people worldwide having disabling hearing loss~\cite{who}.
%
While the focus of this paper is on American sign language translation, since our approach is generic at modeling signs expressed by hands, it can be leveraged for developing sign language translation technologies for potentially any of the three hundred sign languages in use around the world~\cite{signlanguagelist}.
%
Given its promising performance, we believe {\sysname} represents a significant step towards breaking the communication barrier between deaf people and hearing majority, and thus has the significant potential to fundamentally change deaf people's lives.
%It enables millions of deaf people to naturally communicate with others on a day-to-day basis, and thus has the significant potential to fundamentally change deaf people's lives.
%It enables millions of deaf people to naturally communicate with others on a day-to-day basis, and thus has the significant potential to fundamentally change the way deaf people's lives live.












==> ASL_CR - Copy/overview.tex <==
%!TEX root = sensys2017.tex



\section{System Overview}
\label{sec.overview}
\noindent
%In this section, we provide an overview of the system architecture of {\sysname}. 
%
%We then describe two motivating usage scenarios of {\sysname}, both aiming to meet the needs of deaf people in their daily life.
%, with one on teaching ASL and the other on enabling nature communication between a deaf person and people with normal hearing ability.
%%
%\subsection{System Architecture}
%
Figure~\ref{dia.sys} provides an overview of the multi-layer system architecture of {\sysname}.
%that we have designed for recognizing ASL at both word level and sentence level. 
%
Specifically, at the first layer, a temporal sequence of 3D coordinates of the skeleton joints of fingers, palms and forearms is captured by the {\leap} sensor during signing.
% device worn on the chest of a user.
%Gesturing above the sensor results in a sequence of aligned Range-Doppler images which can be thought of as a stream of the dynamics of changing hand configurations (cf. Figure 3, top to bottom).
%
%At the second layer, the key characteristics of ASL signs including finger gesture, hand movement and relative location of two hands are extracted from the 3D coordinates sequence.
At the second layer, the key characteristics of ASL signs including hand shape, hand movement and relative location of two hands are extracted from each frame of the sequence, resulting in a number of spatio-temporal trajectories of ASL characteristics.
%The second layer in the system is the ASL Characteristics Extraction layer where the raw 3D coordinates are de-noised and normalized.
%The output of this layer is the spatio-temporal trajectories of the ASL characteristics.
%The output of this layer is the smoothed and normalized spatio-temporal trajectories of the skeleton joints of fingers, hands and forearms, capturing the hand shapes and movements of the performed ASL.
% 
%Given the spatio-temporal trajectory, 
At the third layer, {\sysname} employs a hierarchical bidirectional deep recurrent neural network (HB-RNN) that models the spatial structure and temporal dynamics of the spatio-temporal trajectories of ASL characteristics for word-level ASL translation.
%At the third layer, {\sysname} employs a hierarchical bidirectional deep recurrent neural network (HB-RNN) that hierarchically transforms the spatio-temporal trajectory of ASL characteristics into an integrated high-level representation for word-level ASL translation.
% for ASL word translation.
%SignSpeak employs a novel hierarchical bidirectional deep recurrent neural network (HB-RNN) to e ectively combine the isolated and unorga- nized low-level ASL characteristics into an integrated high-level representation for word-level ASL translation
%The HB-RNN hierarchically combines the finger gesture, hand movements, and relative locations of two hands to perform ASL translation at the word level.
%
Finally, at the top layer, {\sysname} adopts a CTC-based framework that leverages the captured probabilistic dependencies between words in one complete sentence and translates the whole sentence end-to-end without requiring users to pause between adjacent signs.
%without segmenting the sentence into individual words.
%To address this challenge, we propose to adopt a framework based on Connectionist Temporal Classification (CTC) that removes the requirement of pre-segmentation and thus enables translating the whole sentence end-to-end directly.
%Finally, at the top layer, {\sysname} adopts a probabilistic framework based on Connectionist Temporal Classification (CTC) that leverages the captured probabilistic dependencies between words in one complete sentence to translate the whole sentence end-to-end without segmenting the sentence into individual words.
%
In the next section, we describe the design of {\sysname} in details.
%In the next section, we describe the design of each layer in {\sysname} illustrated in Figure~\ref{dia.sys} in details.

%In particular, it has the advantage of eliminating the effort of segmenting the whole sentence into individual words, and thus translating the whole sentence end-to-end directly.

%% Overview
% 1. draw the system architecture diagram of {\sysname} 
% 2. briefly describe each component within the architecture in the diagram, AND explain how our system solve the challenges listed in the previous section.
%%
% Tutor mode: key idea is hierarchical modeling: we look at each hand and combine them together. To achieve this goal, we first do the pre-processing, and then use LSTM to combine info together in a hierarchical manner.

\begin{figure}[t]
\centering
\includegraphics[scale=0.37]{Images/overview/architecture.pdf}
\caption{The system architecture of {\sysname}.}
\vspace{-4mm}
\label{dia.sys}
\end{figure} 







==> ASL_CR - Copy/related.tex <==
%!TEX root = sensys2017.tex

\section{Related Work}
\label{sec.rw}

%%
\noindent
%Our work is related to prior art in sign language translation systems, and more broadly, mobile sensing systems.
%(2) gesture recognition systems; and most specifically (3) sign language recognition systems. 
%
Our work is related to two research areas: 1) sign language translation; and more broadly 2) mobile sensing systems. 
%In this section, we provide a brief review of the most relevant work within each area.
%In this section, we provide a brief review of the most relevant work within each area and compare them with {\sysname} to show the unique contributions of our work.



\vspace{1mm}
%%
\noindent
\textbf{Sign Language Translation Systems:}
% 1. Existing signal language recognition systems use accelerometer or EMG which are intrusive, and all focus on word/letter recognition.
% 2. Emphasize our work is the first work that preserves privacy and realizing sentence-level ASL recognition.
%%
Over the past few decades, a variety of sign language translation systems based on various sensing modalities have been developed.
%Prior sign language translation systems can be generally classified into wearable sensor-based, Radio Frequency (RF)-based, RGB camera-based, and Kinect-based systems.
% 
Among them, systems based on wearable sensors have been extensively studied~\cite{kim2008bi, kosmidou2009sign, li2010automatic, li2012sign, wu2015real, tubaiz2015glove, praveen2014sign, abhishek2016glove, kanwal2014assistive}. 
%
These systems use motion sensors, EMG sensors, bend sensors, or their combinations to capture hand movements, muscle activities, or bending of fingers to infer the performed signs.
%5
%However, sensor-based approaches require instrumenting fingers, palms, and forearms of users with sensor devices, making them intrusive and impractical for daily usage.
For example, Wu \textit{et al}. developed a wrist-worn device with onboard motion and EMG sensors which is able to recognize $40$ signs~\cite{wu2015real}. 
%
%However, these approaches require the user to heavily equip her fingers, palms or forearms with sensors, making them intrusive and impractical for daily usage.
%RF-based systems use wireless signals as a sensing mechanism to capture hand movements. 
%Melgarejo \textit{et al}. leveraged the different patterns in Received Signal Strength (RSS) and phase information of a wireless link to recognize $25$ sign languages in a wheelchair or a car environment~\cite{melgarejo2014leveraging}.
%
%Although this contactless sensing mechanism minimizes the intrusiveness, RF-based approaches fail to capture hand shape and hand location information, which is critical for recognizing sign languages.
%
Another widely used sensing modality in sign language translation systems is RGB camera~\cite{starner1998real,zafrulla2010novel,brashear2003using}.
%Researchers also use RGB camera-based systems to recognize sign language because it captures rich information about hand shapes and movement~\cite{starner1998real, zafrulla2010novel, brashear2003using}.
%RGB camera-based systems \cite{starner1998real, zafrulla2010novel, brashear2003using}, on the other hand, are capable to capture rich information about hand shapes and movements without heavily instrumenting users. 
%
For example, Starner \textit{et al}. are able to recognize 40 ASL words using Hidden Markov Model with a hat-mounted RGB camera~\cite{starner1998real}.
%
%However, they suffer from bad performance in poor lighting conditions and the videos/images captured may be considered invasive to the user's privacy.
%
There are also some efforts on designing sign language translation systems based on Microsoft Kinect~\cite{chai2013sign, chai2013visualcomm}.
%Recently, researchers use Microsoft Kinect to recognize sign languages because it provides the capability of capturing fine-grained body posture of the user.
%
As an example, by capturing the skeleton joints of the user body and limbs using Microsoft Kinect, Chai \textit{et al}. are able to recognize Chinese Sign Language by matching the collected skeleton trajectory with gallery trajectories~\cite{chai2013sign}.
%Chai \textit{et al}. developed a user interface tool to facilitate the communication with the aid of Kinect.
%%
Most recently, researchers have started exploring using {\leap} to build sign language translation systems~\cite{chuan2014american,marin2014hand}. 
%In contrast to the above approaches, we use infrared light and skeleton joints information of hands for ASL recognition.
%
However, these systems are very limited in their capabilities in the sense that they can only recognize static ASL signs by capturing hand shape information.
%of an ASL sign and thus impossible to recognize signs that involve movement. 
%Moreover, all ASL signs are captured when {\leap} is put statically on a table. 
%
In contrast, {\sysname} captures both hand shape and movement information so that it is able to recognize dynamic signs that involve movements.
%
Most importantly, compared to all the existing sign language translation systems, {\sysname} is the first framework that enables end-to-end ASL sentence translation.
 
%With coarse description of hand shape, Starner \textit{et al}. are able to recognize 42 ASLs using Hidden Marcov Model (HMM) \cite{starner1998real}. To compensate the missing information of the camera, they later proposed a system that also incorporated motion sensors \cite{zafrulla2010novel, brashear2003using} to recognize sign languages more accurately. Furthermore, to mitigate the need for users to wear sensors, they further evaluated the performance of Microsoft Kinect \cite{kinect} in recognition of ASLs \cite{zafrulla2011american}. Similar systems are proposed using Kinect \cite{dominio2014combining, pigou2014sign}. Uebersax et al. used a time-of-flight depth camera to recognize 26 alphabet ASLs \cite{uebersax2011real}. They relax the constraint of proper light condition when performing ASLs by using only depth camera, but the assumption that hands are always the closest objects to the camera deteriorated its practicality. 



%Since its release in 2013, {\leap} has drawn a lot attention in sign language recognition. Chuan et al. used {\leap} API extracted features (e.g., hand grab strength, pointing angles of fingers) and machine learning algorithms k-nearest neighbor (KNN) and support vector machine (SVM) to classify 26 alphabet ASLs \cite{chuan2014american}. Elons et al. used positions and directions of ten finger as the input of a multi-layer perceptron (MLP) to classify 50 Arabic Sign Language (ArSL) gesture \cite{elons2014arabic}. Similarly, Mohandes et al. used 12 features (e.g, finger length, width), and MLP and Naive Bayes Classifier (NBC) to recognize 28 ArSL for Arabic alphabets. Marlin et al. incorporated features extracted from {\leap} with depth and color features from Kinect to recognize ten ASL gestures \cite{marin2014hand}.  However, in these works, the datasets are collected in a very controlled environment. In sum, they made three strong assumptions in collecting and classifying different sign languages: (1) the performed gestures are stationary; (2) the lengths of each gesture are equal; and (3) the collected gesture data is pre-segmented. Furthermore, \cite{elons2014arabic, mohandes2014arabic} used the positions of fingers relative to {\leap} as part of features, assuming that sign languages are always performed at similar locations. Such assumptions might bring serious problems in ASL recognition in the real world environment. 

%Apart from {\leap}, there are numerous other sensing modalities that are capable of recognizing sign languages. In summary, there are three major types of sensing modalities: (1)  sensor based (e.g., electromyography (EMG), motion sensor, sensor gloves); (2) vision based (e.g., depth, RGB camera); and (3) radio-frequency (RF) based. 

%enjoy robust performance in recognizing gestures due to its proximity to the hands. For example, EMG and motion sensor could be combined to serve as a forearm muscle activity indicator in order to capture gestures \cite{kim2008bi, kosmidou2009sign, li2010automatic, li2012sign, wu2015real}. Meanwhile, the sensor gloves, with embedded motion and electric sensors, are capable of capturing the amount of bend, speed and orientation of each finger, and therefore recognizing gestures \cite{tubaiz2015glove, praveen2014sign, abhishek2016glove, kanwal2014assistive}.

%Leveraging the unique impact from a certain hand movement on channel state information (CSI) between the transmitter and receiver antenna pair, RF based sign language recognition system was also proposed to recognize ASL \cite{melgarejo2014leveraging}. RF based approach enjoys the benefit of being non-intrusive and privacy-preserving but is extremely sensitive to background movement and thus could be impractical in the real world environment.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
% TPC: Fred Jiang, Tam Vu, Pei Zhang, Yanyong Zhang, Polly Huang, Tarek, Nic, Jie Liu, Cecilia, Jacob Sorber, John Stankovic, Anthony Rowe, Wen Hu, Octav Chipara, Pengyu Zhang

%
\vspace{1mm}
%%
\noindent
\textbf{Mobile Sensing Systems:}
% 1. Summarize all the sensing modalities explored in the existing systems.
% 2. Emphasize our work is the first work that explores infrared sensing in the context of ASL recognition. With the incoming AR/VR headsets, we envision infrared sensing will be part of the future mobile and wearable sensing systems.
%The past few years have witnessed the surge of wearable devices. 
%Researchers have developed a variety of wearable sensing systems based on various sensing modalities for monitoring user behaviors, measuring vital signs, and providing new mechanisms for human-computer interaction.
%
Our work is also broadly related to research in mobile sensing systems.
%
Prior mobile sensing systems have explored a variety of sensing modalities that have enabled a wide range of innovative applications.
%
Among them, accelerometer, microphone and physiological sensors are some of the mostly explored sensing modalities.
%
For example, Mokaya \textit{et al.} developed an accelerometer-based system to sense skeletal muscle vibrations for quantifying skeletal muscle fatigue in an exercise setting \cite{mokaya2016burnout}. 
%Shen \textit{et al.} developed a smartwatch based system to track arm postures \cite{shen2016smartwatch}.
%
Nirjon \textit{et al.} developed MusicalHeart \cite{nirjon2012musicalheart} which integrated a microphone into an earphone to extract heartbeat information from audio signals.
%
Nguyen \textit{et al.} designed an in-ear sensing system in the form of earplugs that is able to capture EEG, EOG, and EMG signals for sleep monitoring \cite{nguyen2016lightweight}.
%
Recently, researchers have started exploring using wireless radio signal as a contactless sensing mechanism. 
%
For example, Wang \textit{et al.} developed WiFall \cite{wang2017wifall} that used wireless radio signal to detect accidental falls.
%
Fang \textit{et al.} used radio as a single sensing modality for integrated activities of daily living and vital sign monitoring \cite{fang2016bodyscan}.
%
In this work, we explore infrared light as a new sensing modality in the context of ASL translation.
%
It complements existing mobile sensing systems by providing a non-intrusive and high-resolution sensing scheme.
%, with no constraint of ambient lighting conditions.
%
We regard this work as an excellent example to demonstrate the usefulness of infrared sensing for mobile systems.
%
With the incoming era of virtual/augmented reality, we envision infrared sensing will be integrated into many future mobile systems such as smartphones and smart glasses.
%We envision that infrared cameras will be integrated into future wearables and mobile devices such as AR/VR headsets to enable natural interaction. 

%\vspace{1mm}
%%
%\noindent
%\textbf{Gesture Recognition Systems:}
% 1. Existing gesture recognition systems, no matter what sensing modalities are being used, all focus on very simple, small, self-defined set of gestures.
% 2. Emphasize sign language is way more complicated than general gestures, and requires sensing modality that can provide high resolution to capture the hand-shape and movements.
 










